Coarser Equivalences for Causal Concurrency

Trace theory is a principled framework for defining equivalence relations for concurrent program runs based on a commutativity relation over the set of atomic steps taken by individual program threads. Its simplicity, elegance, and algorithmic efficiency makes it useful in many different contexts including program verification and testing. We study relaxations of trace equivalence with the goal of maintaining its algorithmic advantages. We first prove that the largest appropriate relaxation of trace equivalence, an equivalence relation that preserves the order of steps taken by each thread and what write operation each read operation observes, does not yield efficient algorithms. We prove a linear space lower bound for the problem of checking, in a streaming setting, if two arbitrary steps of a concurrent program run are causally concurrent (i.e. they can be reordered in an equivalent run) or causally ordered (i.e. they always appear in the same order in all equivalent runs). The same problem can be decided in constant space for trace equivalence. Next, we propose a new commutativity-based notion of equivalence called grain equivalence that is strictly more relaxed than trace equivalence, and yet yields a constant space algorithm for the same problem. This notion of equivalence uses commutativity of grains, which are sequences of atomic steps, in addition to the standard commutativity from trace theory. We study the two distinct cases when the grains are contiguous subwords of the input program run and when they are not, formulate the precise definition of causal concurrency in each case, and show that they can be decided in constant space, despite being strict relaxations of the notion of causal concurrency based on trace equivalence.

==> algorithm-check-order.tex <==
%!TEX root=./main.tex

\section{Checking Causal Concurrency Under Block Swaps}\label{sec:alg-co}

We now turn our attention to the algorithmic aspects
of the coarser notion of block equivalence we introduced
in \secref{bpo}.
% As before, we focus our attention on checking causal concurrency
% between events, under the equivalence $\ofbeq$.
% We will show that the predicate $\checkConc{\ofbeq}{\cdot}{\cdot}{\cdot}$
% can be determined using an algorithm thar runs in 
% a streaming one pass fashion and uses only constant space
% (assuming the number of threads $|\threads|$ and variables $|\vars|$
% is constant).
We will show that causal concurrency between two given events
in a program run can be determined using an algorithm thar runs in 
a streaming one pass fashion and uses constant space
(assuming the alphabet $\alphabet_\noval$ has $O(1)$ size).

% \myparagraph{Overview of the algorithm}{
% Our algorithm stems out of the following high level insights.
% First, given a set of a blocks $\blocks$, we show that the
% induced saturated partial order $\bhbs$ can be monitored using constant space.
% That is, there is a constant space algorithm that, given an
% execution appearing as a stream of events, together with the position of an event $e$
% in the execution, tracks and updates summary information about $e$
% that can be used to determine, for every event $e'$ appearing in the execution,
% whether $e \bhbs e'$, at the time of occurrence of $e'$ in the stream.
% We present this algorithm in \ucomment{section}.
% Second, we show that this monitoring algorithm can also
% be used to design a constant space algorithm for determine
% liberal atomicity for the choice of blocks $\blocks$ under consideration.
% This is presented in \ucomment{section}.
% The two algorithms thus far can then be put together to
% show that, given a set of blocks $\blocks$,
% checking causal concurrency under block swaps restricted to blocks in $\blocks$,
% is solvable using a constant space algorithm.
% We extend this algorithm to finally develop, \ucomment{in section ...} a constant space algorithm 
% for checking causal concurrency under the \orclFreeBlkTextSmall equivalence, as defined in \secref{select-blocks}.
% }

\myparagraph{Overview of the algorithm}{
	Our algorithm stems from the following high level insights.
	First, given a set of a blocks $\blocks$, we show, in \secref{algo-track-bhbs}, that the
	induced saturated partial order $\bhbs$ can be tracked using constant space,
	independent of whether $\blocks$ is liberally atomic or not.
	By tracking the partial order, we mean that, given a fixed
	event $e$ in the execution, we can determine  
	if $e \bhbs e'$ for any given event $e'$, by only keeping constant amount of memory when traversing the
	execution in a streaming fashion.
	We remark that, even though the partial order $\bhb$ and its saturated version $\bhbs$,
	are defined for a set of liberally atomic blocks $\blocks$ (\defref{bhb}),
	the assumption on liberal atomicity is only required for ensuring soundness (\thmref{soundness}).
	Our algorithm does not, in principle, require the assumption of liberal atomicity.
	Second, we show that the algorithm for tracking $\bhbs$, in fact, can be used
	to design a constant space algorithm
	for checking liberal atomicity of $\blocks$ (\secref{la-alg}).
	The ideas behind this algorithm are inspired by~\cite{FM08CAV}, 
	in which the authors design a constant space
	algorithm for checking \emph{conflict serializability}.
	Together, we get a sound and complete algorithm for checking causal concurrency
	under the equivalence induced by a given set of $\blocks$.
	We finally consider an even weaker notion of equivalence
	(\secref{select-blocks}) where we ask `are the two given events causally concurrent
	under some choice of blocks?'. We show that this more general concurrency
	criterion can also be monitored  using a constant space streaming algorithm.
}

\begin{comment}
\subsection{Overview of the algorithm}

	Overall, our approach is as follows.
	We start by tackling the problem of checking causal concurrency 
	under the equivalence $\fbeq$,
	for a given set of liberally atomic blocks $\blocks$.
	To achieve this, we resort to the
	partial order $\bhbs$ induced by $\blocks$ and use its
	correspondence with the equivalence $\fbeq$ relation, as in~\thmref{coincidence}
	and \thmref{soundness}.

	Our first algorithmic result in this context is the following.
	Given a set of a blocks $\blocks$ in an execution $w$, we show that the
	induced saturated partial order $\bhbs$ can be \emph{tracked} using only constant space.
	By tracking the partial order, we mean that, given a fixed
	event $e$ in the execution, we can determine, for every later event $e'$, 
	if $e \bhbs e'$ by only keeping constant amount of memory when traversing the
	execution in a streaming fashion.
	This algorithm is presented in \secref{algo-track-bhbs}.

	We next turn our attention to the \orclFreeBlkTextSmall equivalence $\ofbeq$ and the corresponding
	question $\checkConc{\ofbeq}{\cdot}{\cdot}{\cdot}$.
	In this notion of equivalence, we do not have
	a given set of liberally atomic $\blocks$ at our disposal, 
	and need to consider all selections of liberally atomic blocks.
	Our approach here is to \emph{enumerate} the set of 
	blocks $\block$, and \emph{check} if the guessed set $\blocks$ is 
	(a) liberally atomic, and (b) induces an equivalence $\fbeq$ for which
	the two given events are causally concurrent.
	This procedure can, in principle be expensive and may lead to an inefficient overall algorithm.
	This is where we rely on our earlier algorithm (\secref{algo-track-bhbs})  
	for tracking $\bhbs$ in constant space.
	Since a constant space algorithm corresponds to a finite state automaton,
	we can wield the power of \emph{non-determinism} to get an overall
	constant space algorithm for tracking all the partial orders
	induced by all selections of blocks, while still staying in the realm 
	of a constant space algorithm.
	In essence, we build a non-deterministic finite state automaton that 
	\emph{guesses} the choice of blocks, and \emph{checks} if the choice
	is liberally atomic and can be used to conclude concurrency between events. 

	The first remaining ingredient in our guess-and-check scheme is the problem
	of determining if a given guess for the choice of blocks $\blocks$ is liberally atomic.
	We show that a constant space algorithm for tracking the partial order
	induced by $\blocks$ also lends itself to a constant space algorithm
	for checking liberal atomicity of $\blocks$.
	The ideas behind this algorithm are inspired from~\cite{FM08CAV}
	where the authors design a constant space
	algorithm for checking \emph{conflict serializability}.
	Conflict serializability is a stronger notion 
	than liberal atomicity
	and corresponds to the case when $\blocks = \emptyset$, 
	in which case the corresponding equivalence is Mazurkiewicz equivalence ($\hb$).
	We generalize these ideas for checking liberal atomicity, given a choice of candidate $\blocks$
	and present a constant space algorithm in \ucomment{section}, 
	based on the algorithm in \secref{algo-track-bhbs}.

	The second task in our guess-and-check scheme is to efficiently guess the blocks.
	We do this using standard automata-theoretic techniques and present
	the overall constant-space algorithm in \ucomment{section}.
\end{comment}

\input{block-partial-order-algo}
\input{liberal-atomicity-algo}
\input{cc-block-algo}
\input{block-selection}

==> app-algo.tex <==
% !TEX root = main.tex
\section{Proofs of Theorems in \secref{alg-co}}

\subsection{Proof of \thmref{liberal-atomicity-cycle}}

\begin{proof}
($\Rightarrow$) Consider the case when $G_\blocks$ is cyclic.
Then there are distinct nodes $n_0, \ldots, n_{k-1} \in V_\blocks$ (with $k \geq 2$) 
and events $e_0, f_0 \in n_0$, $e_1, f_1 \in n_1 \ldots, e_{k-1}, f_{k-1} \in n_{k-1}$
such that
$f_{i-1} \bhbs e_{i\%k}$ for every $i \in \range{k}$.
Assume, for the sake of contradiction that there is a string $w'$
such that $w'$ is serial (i.e., all blocks appear contiguously in $w'$)
and $w' \fbeq w$.
By \thmref{soundness}, we must have that $f_{i-1}$ occurs before $e_{i\%k}$
in $w'$ for each $i \in \range{k}$.
Since all blocks occur contiguously in $w'$, we must also have that
both $e_{i-1}$ and $f_{i-1}$ occur before 
both $e_{i\%k}$ and $f_{i\%k}$ in $w'$, for every $i$.
This means that $e_0$ occurs before $e_1$ and $e_1$ occus before $e_0$ in $w'$,
which is a contradiction.

($\Leftarrow$)
Let $\graph_\blocks$ be acyclic. 
Then we will show that we can construct a
proper linearization $w'$ of $\bhbs$
(using an algorithm similar to that in \thmref{tsort})
in which all blocks are contiguous.
For this, we first consider the directed graph $G_w = (V_w, E_w)$,
where $V_w$ is the set of events and
the set of edges
$E_w = \setpred{(e_1, e_2)}{\exists n_1, n_2 \in V_\blocks, e_1 \in n_1, e_2 \in n_2, (n_1, n_2) \in E_\blocks}$ 
is inferred from the block graph $G_\blocks$.
First, we claim that $G_w$ is acyclic.
This is because a cycle $e_0, e_1, \ldots, e_{k-1}$ in $G_w$ implies
that the corresponding sequence of nodes $n_0, n_1, \ldots, n_k$
also form a cycle in $G_\blocks$.
Next, we claim that the following 
steps produce a proper linearization of the set of events $V_w$ of
$E_w$, and thus a linearization of $\bhbs$ (since $\bhbs \subseteq E_w^+$).
\begin{enumerate}
\item Start with $v = \epsilon$.
\item Let $e \in V_w$ such that $\not \exists f \in V_w:\ (f, e) \in E_w$ and 
if $\OpOf{e} = \rd$, then $\VariableOf{e}$ is not the same as the variable of any open block in $v$. 
\item Set $V_w = V_w - \set{e}$ and $v = ve$.
\item If $V_w \neq \emptyset$, then go to (2).
\end{enumerate}
The proof of correctness of the algorithm is similar to that
of \thmref{tsort} and thus skipped. 
%\ucomment{should we skip this?}
\end{proof}


==> app-automata.tex <==
%!TEX root = ./main.tex

\section{Detailed description of the Saturation Automaton}
\applabel{app-automata}

The components of our \underline{sat}uration automaton are
\[\autsup{\saturated} = (\statessup{\saturated}, \initsup{\saturated}, \transsup{\saturated})\]
where $\statessup{\saturated}$ is the set of states,
$\initsup{\saturated} \in \statessup{\saturated}$ is a dedicated initial state
and $\transsup{\saturated} : \statessup{\saturated} \times \extendBlk{\alphabet}_\noval \to \statessup{\saturated}$
is the transition function. 
We next describe each of these in detail.

\myparagraph{\it \underline{States of $\autsup{\saturated}$}}{
	Each state $q \in \statessup{\saturated}$ is a tuple of the form
	\[
		q = (\autBlks, \autRF, \autAfterSat, \autBlkAfter, \autBlkAfterOpen)
	\]
	where,
	\begin{itemize}
		\item $\autBlks : \vars \partialto \powset{\extendBlk{\alphabet}_\noval}$
		maps each variable $x \in \vars$ to the contents of the running block $B_x$ on variable $x$
		in the execution seen so far. If no such block exists, $\autBlks(x) = \emptyset$,

		\item $\autRF : \vars \partialto \extendBlk{\alphabet}_\noval$ maps each variable $x$
		to the label of the last write on $x$. This will be used to track the reads-from dependency
		for read events,

		\item $\autAfterSat : \extendBlk{\alphabet}_\noval \to \powset{\extendBlk{\alphabet}_\noval}$
		maps each symbol $a \in \extendBlk{\alphabet}_\noval$ to the after set $\after{\bhbseq}(e_a)$
		induced by the saturated order $\bhbseq$,
		where $e_a$ is the last event with label $a$,

		\item The map $\autBlkAfter : \extendBlk{\alphabet}_\noval \times \threads \times \vars \to \powset{\extendBlk{\alphabet}_\noval}$ is such that
		for each symbol $a \in \extendBlk{\alphabet}_\noval$,
		thread $t$ and variable $x$, $\autBlkAfter(a, t, x)$
		stores the $\bhbseq$-after set of the first block $B_{t,x}$ such that
		$\ThreadOf{B} = t$, $\VariableOf{B} = x$, and
		there is an event $e \in B_{t,x}$ such that $e_a \bhbseq e$;
		here $e_a$ is the latest event with label $a$.
		
		\item Finally, $\autBlkAfterOpen : \extendBlk{\alphabet}_\noval \times \threads \times \vars \to \set{\tru, \fls}$ is such that $\autBlkAfterOpen(a, t, x)$  
		tracks if the block $B_{t,x}$ defined above is currently open.
	\end{itemize}
	The components of a given state $q$ will be refered to as $q.\autBlks$, $q.\autRF$, $q.\autAfterSat$ and $q.\autBlkAfter$.
}

\myparagraph{\it \underline{Initial State of $\autsup{\saturated}$}}{
	The initial state $\initsup{\saturated} \in \statessup{\saturated}$
	is such that
	$\autRF(x) = \undf$,
	 $\autBlks(x) =  \autAfterSat(a) = \autBlkAfter(a,t,x) = \emptyset$,
	and, $\autBlkAfterOpen(a, t,x) = \top$ for each $a \in \extendBlk{\alphabet}_\noval$, $t \in \threads$ and $x \in \vars$.
}

\myparagraph{\it \underline{Transitions of $\autsup{\saturated}$}}{
	The transitions of the automaton are detailed, but intuitive.
	For a given $q \in \statessup{\saturated}$ and symbol $a \in \extendBlk{\alphabet}_\noval$,
	we describe the components of the state $q' = \transsup{\saturated}(q, a)$ below.
	\begin{description}
		\item[$\autBlks$.] For every variable $z$, the set $q'.\autBlks(z)$ is either the same as in $q$,
		an emptyset, or the contents of the block it participates in:
		 \[
			q'.\autBlks(z) = \begin{cases}
			\set{a} & \text{ if } z = x, \OpOf{a} = \wt, \text{ and } \AnnotOf{a} = \top \\
			q.\autBlks(x) \cup \set{a} & \text{ if } z = x, \OpOf{a} = \rd, \text{ and } \AnnotOf{a} = \top \\
			\emptyset & \text{ if } z = x \text{ and } \AnnotOf{a} = \bot \\
			q.\autBlks(z) & \text{ if } z \neq x
			\end{cases}
		\]

		\item[$\autRF$.] The function $\autRF$ is updated in the most natural manner:
		\[
			q'.\autRF(z) = \begin{cases}
			a & \text{ if } z = x, \text{ and } \OpOf{a} = \wt \\
			q.\autRF(z) & \text{ otherwise }
			\end{cases}
		\]

		\item[$\autAfterSat$ and $\autBlkAfter$.] 
		The updates to the maps $\autAfterSat$ and $\autBlkAfter$
		are a bit more involved.
		Let us understand why.
		Suppose there is a symbol $c$ such that $a$ induces a $\bhbeq$ dependency 
		with some $a' \in \autAfterSat(c)$.
		Then, $a$ should be added to $\autAfterSat(c)$.
		This in turn menas that $a'$ should also be added to
		$\autBlkAfter(c', t, x)$ if it contains $c$.
		More importantly, if the first block $B_{t,x}$ $\bhbseq$-after $c'$
		is closed and $\VariableOf{a} = x$, then $a$ must also be
		added to $\autAfterSat(c')$.
		This chain of reasoning can continue even further.
		In view of this, we present a least fixpoint style
		formulation for the new maps $q'.\autAfterSat$ and $q'.\autBlkAfter$.

		% Let us now describe the fixpoint definitions of the
		% components $\autAfterSat$ and $\autBlkAfter$ in the new state $q'$.
		We define sets $\setpred{A_c}{c \in \extendBlk{\alphabet}_\noval}$ and 
		$\setpred{FBA_{c, t, x}}{c \in \extendBlk{\alphabet}_\noval, t \in \threads, x \in \vars}$ as the smallest
		sets that satisfy the following conditions:
		% \begin{enumerate}[label=(\arabic*)]
		% 	\item For every $c$, $\deprf(a) \cap A_c \implies a \in A_c$.
		% 	\item For every $c$, $q.\autAfterSat(c) \subseteq A_c$.
		% 	\item For every $c, t, x$, $q.\autBlkAfter(c, t, x) \subseteq FBA_{c, t, x}$.
		% 	\item For every $c, d$, $\deprf(d) \cap A_c \implies A_d \subseteq A_c$.
		% 	\item For every $c, t, x, d$, $\deprf(d) \cap FBA_{c, t, x} \implies A_d \subseteq FBA_{c, t, x}$.
		% 	\item For every $c, d \in \extendBlk{\alphabet}_\noval$ with
		% 	$t = \ThreadOf{d}$, $x = \VariableOf{d}$ and $\AnnotOf{d} = \top$:
		% 	\[
		% 	q.\autBlkAfter(c, t, x) = \emptyset \land d \in A_c \implies 
		% 	\forall d' \in q'.\autBlks(x), A_{d'} \subseteq FBA_{c, t, x}
		% 	\]
		% 	\item For every $c, d \in \extendBlk{\alphabet}_\noval$ with 
		% 	$t = \ThreadOf{d}$, $x = \VariableOf{d}$ and $\AnnotOf{d} = \top$:
		% 	\[
		% 	q.\autBlkAfterOpen(c, t, x) = \bot \land d \in FBA_{c, t, x} \implies 
		% 	A_d \subseteq A_c
		% 	\]
		% \end{enumerate}
		\begin{align*}
		\begin{array}{rl}
			\deprf(a) \cap A_c \implies a \in A_c & \text{ for every } c \\[0.5em]
			q.\autAfterSat(c) \subseteq A_c & \text{ for every } c \\[0.5em]
			q.\autBlkAfter(c, t, x) \subseteq FBA_{c, t, x} & \text{ for every } c, t, x \\[0.5em]
			\deprf(d) \cap A_c \implies A_d \subseteq A_c & \text{ for every } c, d \\[0.5em]
			\deprf(d) \cap FBA_{c, t, x} \implies A_d \subseteq FBA_{c, t, x} & \text{ for every } c, t, x, d \\[0.5em]
			\!\!\!\begin{array}{l}
			d \in A_c %\\
			\land \, q.\autBlkAfter(c, t, x) = \emptyset %\\
			% \land \, d \in A_c
			\end{array}\!\!
			{\implies} 
			A_{d'} \subseteq FBA_{c, t, x} 
			&\!\!\!\begin{array}{l}
			% \text{ for every } c, d, d' \text{ with } t = \ThreadOf{d}, \\
			% \,x = \VariableOf{d}, \AnnotOf{d} = \top, d' \in q'.\autBlks(x)
			\text{ for every } c, d, d', t, x, \text{ with } t = \ThreadOf{d}, \\
			\,x = \VariableOf{d}, 
			\AnnotOf{d} = \top, d' \in q'.\autBlks(x)
			\end{array} \\[1em]
			\!\!\!\begin{array}{c}
			d \in FBA_{c, t, x} %\\
			\land \, q.\autBlkAfterOpen(c, t, x) = \bot 
			\end{array}\!\!
			{\implies} 
			A_d \subseteq A_c
			&\!\!\!\begin{array}{l}
			% \text{ for every } c, d, \text{ with } t = \ThreadOf{d}, \\
			% \,x = \VariableOf{d}, \AnnotOf{d} = \top
			\text{ for every } c, d, t, x \text{ with } t = \ThreadOf{d}, \\
			\,x = \VariableOf{d}, \AnnotOf{d} = \top
			\end{array}
		\end{array}
		\end{align*}
		Here, for a symbol $c \in \extendBlk{\alphabet}_\noval$,
		we use the notation: 
		\[
		\annotDep = \deprel_\noval \times \set{\top, \bot} \setminus \setpred{(a, b)}{\ThreadOf{a} \neq \ThreadOf{b} \text{ and } \bot \not\in \set{\AnnotOf{a}, \AnnotOf{b}}}
		\]
		\[\deprf(c) = 
		\begin{cases}
			\setpred{c'}{(c, c') \in \annotDep} & \text{ if } \OpOf{c} = \wt \\
			\setpred{c'}{\set{(c, c'), (c_{\rdf{}}, c')} \cap \annotDep \neq \emptyset} & \text{ otherwise if } \OpOf{c} = \rd \text{ and } c_{\rdf{}} = q.\autRF(\VariableOf{c})
		\end{cases}
		\]
		We remark that the sets $\setpred{A_c}{c \in \extendBlk{\alphabet}_\noval}$
		and $\setpred{FBA_{c,t,x}}{c \in \extendBlk{\alphabet}_\noval, t\in\threads, x \in\vars}$ can be computed in an iterative manner
		in time that is linear in 
		the size of a state $O(|\extendBlk{\alphabet}_\noval|{\cdot}|\threads|{\cdot}|\vars|)$ 
		which is a constant.

		Having defined these fixpoint sets, we can now define $q'.\autAfterSat$ and $q'.\autBlkAfter$ as follows. 
		First, for every $c \in \extendBlk{\alphabet}_\noval$,
		\[
			q'.\autAfterSat(c) = \begin{cases}
				\set{a} & \text{ if } c = a\\
			A_c & \text{ otherwise }
			\end{cases}
		\]

		The sets $q'.\autBlkAfter$ are described as follows.
		For a symbol $c \in \extendBlk{\alphabet}_\noval$, thread $t\in \threads$
		and variable $x \in \vars$, we have
		\[
			q'.\autBlkAfter(c, t, x) = 
			\begin{cases}
				\set{a} 
				& 
				\text{ if } 
				\begin{array}{l}
				c = a, \AnnotOf{a} = \top, \VariableOf{a} = x, \\
				\OpOf{a} = \wt, \ThreadOf{a} = t
				\end{array} \\
				A_{a_{\rdf{}}} 
				&
				\text{ if } 
				\begin{array}{l}\AnnotOf{a} = \top, \VariableOf{a} = x, \OpOf{a} = \rd, \\
				a_{\rdf{}} = q.\autRF(a), \ThreadOf{a_{\rdf{}}} = t
				\end{array}\\
				\emptyset
				&
				\text{ otherwise if } a = c \\
				FBA_{c, t, x}
				&
				\text{ otherwise}
			\end{cases}
		\]
		\begin{comment}
		Next, the sets $q'.\autBlkAfter$ corresponding to the input symbol $a$ 
		are described as follows.
		For thread $t \in \threads$ and variable $x \in \vars$,
		\[
			q'.\autBlkAfter(a, t, x) = 
			\begin{cases}
				\set{a} 
				& 
				\text{ if } 
				\begin{array}{l}
				\AnnotOf{a} = \top, \VariableOf{a} = x, \\
				\OpOf{a} = \wt, \ThreadOf{a} = t
				\end{array} \\
				A_{a_{\rdf{}}} 
				&
				\text{ if } 
				\begin{array}{l}\AnnotOf{a} = \top, \VariableOf{a} = x, \OpOf{a} = \rd, \\
				a_{\rdf{}} = q.\autRF(a), \ThreadOf{a_{\rdf{}}} = t
				\end{array}\\
				\emptyset
				&
				\text{ otherwise }
			\end{cases}
		\]

		Finally, for a symbol $c \neq a$, thread $t$ and variable $x$,
		\[
		q'.\autBlkAfter(c, t, x) = FBA_{c, t, x}
		\]
		\end{comment}

		\item[$\autBlkAfterOpen$.] 
		First, for the input symbol $a$, the
		only blocks $\bhbseq$-after the current event $e_a$ labeled with $a$ 
		are those that $e_a$ is a part of, and thus they must be open.
		% \[
		% 	q'.\autBlkAfterOpen(a, t, x) = \top \text{ for every } t\in \threads, x \in \vars.
		% \]
		For any other symbol, 
		we must declare the fist block that is $\bhbseq$-after the symbol to be closed,
		if the input $a$ starts a new block on the same variable as the block.
		That is, for $c \in \extendBlk{\alphabet}_\noval$, $t \in \threads$
		and $x \in \vars$,
		\[
			q'.\autBlkAfterOpen(c, t, x) = \begin{cases}
				\top
				&
				\text{ if } c = a \\
				\bot 
				& 
				\text{ if } 
				\begin{array}{l}
				c \neq a, \AnnotOf{a} = \top, \VariableOf{a} = x, \OpOf{a} = \wt, \\
				\text{ and } q.\autBlkAfterOpen(c, t, x) \neq \emptyset
				\end{array}\\
				q.\autBlkAfterOpen(c, t, x)
				&
				\text{ otherwise }
			\end{cases}
		\]
	\end{description}
}


This concludes the description of the automaton $\autsup{\saturated}$.
We now state the key invariant useful for designing later algorithms.

\begin{theorem}
\thmlabel{automata-saturation-invariant-strong}
Let $\tr \in \alphabet_\noval^+$, $\blocks$ be a set of blocks in $\tr$
and let $\extendBlk{\tr} \in \extendBlk{\alphabet}_\noval^*$ be the corresponding annotated execution.
Let $q = \transsup{\saturated}^*(\initsup{\saturated}, \extendBlk{\tr})$
be the state reached by the automaton $\autsup{\saturated}$ on the string $\extendBlk{\tr}$.
For each $a \in \extendBlk{\alphabet}_\noval$, let $e_a$ be the last event in 
$\extendBlk{\tr}$ such that $\extendBlk{\tr}[e_a] = a$.
For each variable $x \in \vars$, let $B_x \in \blocks$ be the last block $B$ with $\VariableOf{B} = x$
in $\tr$ ($B_x = \emptyset$ if no such block exists).
Then, we have the following.
\begin{description}[labelindent=0.5cm]
	\item[Inv-$\autBlks$.]
		For every $x \in \vars$, $q.\autBlks(x) = \setpred{\extendBlk{\tr}[e]}{e \in B_x}$
	\item[Inv-$\autRF$.]
		For every $a \in \extendBlk{\alphabet}_\noval$, 
		$q.\autRF(a) = \extendBlk{\tr}[\rdf{e_a}]$, if $\OpOf{a} = \rd$ and $e_a$ exists;
		otherwise,  $q.\autRF(a) = \undf$.
	\item[Inv-$\autAfterSat$.] 
		For every $a \in \extendBlk{\alphabet}_\noval$,
		$q.\autAfterSat(a) = \after{\bhbseq}(e_a)$ if $e_a$ exists; and $\emptyset$ otherwise.
	\item[Inv-$\autBlkAfter$.] 
		For every $a \in \extendBlk{\alphabet}_\noval$, $t \in \threads$, $x \in \vars$,
		$q.\autBlkAfter(a, t, x) = \fstblkafter{\bhbeq}{t}{x}(e_a)$ if $e_a$ exists;
		otherwise $q.\autBlkAfter(a, t, x) = \emptyset$.
	\item[Inv-$\autBlkAfterOpen$.]
		For every $a \in \extendBlk{\alphabet}_\noval$, $t \in \threads$, $x \in \vars$,
		$q.\autBlkAfterOpen(a, t, x) = \bot$ if $e_a$ exists, and there are at least two blocks
		$B_1 \neq B_2 \in \blocks$ such that $\VariableOf{B_1} = \VariableOf{B_1} = x$,
		$\ThreadOf{B_1} = \ThreadOf{B_2} = t$, $\exists i_1 \in B_1, e_a \bhbseq i_1$, 
		and $\exists i_2 \in B_2, e_a \bhbseq i_2$;
		otherwise, $q.\autBlkAfterOpen(a, t, x) = \top$.	
\end{description}
\end{theorem}

==> app-semantic-hardness.tex <==
%!TEX root = main.tex

\section{Proofs from \secref{semantic-equivalence}}
\applabel{proofs-semantic-equivalence}

\input{construction-check-order}

==> block-partial-order-algo.tex <==
%!TEX root=./main.tex

\subsection{Tracking Saturated Block Partial Order}
\seclabel{algo-track-bhbs}

% The partial order $\bhb$ and its saturated version $\bhbs$,
% is defined for a set of liberally atomic blocks $\blocks$ (\deflabel{bhb}).
% The assumption on liberal atomicity



\myparagraph{Annotating runs with blocks}{
Let $\tr \in \alphabet_\noval^*$ be a concurrent run and
let $\blocks$ be a set of blocks in $\tr$.
We can annotate $\tr$ with $\blocks$
to get the string $\extendBlk{\tr}$
over the extended alphabet $\extendBlk{\alphabet}_\noval = \alphabet_\noval \times \set{\tru, \fls}$
such that $|\extendBlk{\tr}| = |\tr|$ and for every $i \leq |\tr|$,
$\extendBlk{\tr}[i] = (\tr[i], \top)$ if the event $e_i$ at index $i$
is such that $e_i \in B$ for some $B \in \blocks$, and $\extendBlk{\tr}[i] = (\tr[i], \bot)$ otherwise.
The annotated trace $\extendBlk{\tr}$ is assumed to be on the same set of events as $\tr$, and we will skip formalizing this.
% \[
% \extendBlk{\tr}[i] = 
% \begin{cases}
% (\tr[i], \top) & \text{ if } i \in B, \text{ for some } B \in \blocks \\
% (\tr[i], \bot) & \text{ otherwise}
% \end{cases}
% \]
For an extended symbol $a' = (a, {\sf b}) \in \extendBlk{\alphabet}_\noval$, we will use
the notation $\AnnotOf{a'} = {\sf b}$,
and overload the notations $\ThreadOf{a'} = \ThreadOf{a}$,
$\VariableOf{a'} = \VariableOf{a}$,
$\OpOf{a'} = \OpOf{a}$.
\begin{comment}
Extending the run by providing additional Boolean annotation ($\tru$ or $\fls$)
at every event allows us to give a \emph{syntactic}, almost 
Mazurkiewicz trace like characterization of
$\bhb$.
Extending the execution by providing additional Boolean annotation ($\tru$ or $\fls$)
at every event allows us to give a \emph{syntactic}, almost 
Mazurkiewicz trace like characterization of
$\bhb$.
Let $\extendBlk{\deprel}_\noval = \deprel_\noval \times \set{\tru, \fls}$. 
Consider the dependence relation 
$\extendBlk{\deprel} \subseteq \extendBlk{\alphabet}_\noval \times \extendBlk{\alphabet}_\noval$
defined below. 
\[
\annotDep = \extendBlk{\deprel}_\noval \setminus \setpred{\big((a, \alpha), (b, \beta)\big)}{(a, b) \in \deprel_\noval \text{ and } \top \in \set{\alpha, \beta}}
\]
\begin{proposition}
\proplabel{unroll-annot-bhb}
Let $\tr \in \alphabet_\noval^*$ be a concurrent execution,
$\blocks$ be a set of blocks in $\tr$,
$\extendBlk{\tr} \in \extendBlk{\alphabet}_\noval$ be the corresponding annotated execution,
and let $i \neq j \in \range{|\tr|}$ be two events.
$i \bhb j$ iff there is a sequence of indices
$k_0 < k_1 < \cdots < k_n$ such that $n > 0$ and
\begin{enumerate*}[label=(\alph*)]
	\item $k_0 = i$,
	\item $k_n = j$, and
	\item for every $m < n$, either $k_m = \rdf{w}(k_{m+1})$, or $(\extendBlk{\tr}[k_m], \extendBlk{\tr}[k_{m+1}]) \in \annotDep$.
\end{enumerate*}
\end{proposition}
\end{comment}
}

\myparagraph{After Sets}{
% We now discuss the key ingredient in our constant space algorithm.
% The algorithm relies on succinct representation of 
% the dependencies implied by the partial order $\bhbs$,
% in the form of \emph{after set} which we describe next.
A key ingredient in our constant space algorithm is 
the succinct representation of 
the dependencies implied by the partial order $\bhbs$.
Let us fix an annotated run $\extendBlk{\tr}$
corrresponding to a concurrent run $\tr \in \alphabet_\noval^*$
and set of blocks $\blocks$ in $\tr$.
% and the corresponding annotated execution $\extendBlk{\tr}$.
For an event $e$ of $\tr$,
the $\bhbseq$-after set of $e$ is
\begin{align}
\begin{array}{rcl}
\after{\bhbseq}(e) &=& \setpred{\extendBlk{\tr}[f]}{e \bhbseq f} \\
\end{array}
\end{align}
Here, we use the notation $\bhbseq$ to denote the reflexive closure of $\bhbs$.
Observe that, for any event $e$, $\after{\bhbseq}(e) \subseteq \extendBlk{\alphabet}_\noval$
and thus has constant size.
The following proposition illustrates the correspondence between
the $\bhbseq$-after sets the partial order $\bhbs$.
\begin{proposition}
% Let $\tr \in \alphabet_\noval^*$ be a concurrent execution,
% $\blocks$ be a set of blocks in $\tr$,
% $\extendBlk{\tr} \in \extendBlk{\alphabet}_\noval$ be the corresponding annotated execution.
Let $e, f \in \events{\tr}$ be events such that $e$ appears before $f$ in $\tr$.
Then, $e \bhbs f \text{ iff } \extendBlk{\tr}[f] \in \after{\bhbseq}(e)$
% \[
% i \bhbs j \text{ iff } \extendBlk{\tr}[j] \in \after{\bhbseq}(i)
% \]
\end{proposition}
}

\myparagraph{Efficiently Constructing After Sets}{
The algorithm will essentially maintain the $\bhbseq$-after set
of a given event in a streaming fashion.
In order to do so, we need to track two kinds of dependencies.
The first set of dependencies arise from the fact that
$\bhbseq$ right-composes with $\bhbeq$, the reflexive closure of the unsaturated order $\bhb$. 
Thus, if we have events $e_1, e_2, e_3$ such that
$e_1 \bhbseq e_2$ and $e_2 \bhbeq e_3$, then
we have $e_1 \bhbseq e_3$.
The second set of dependencies arise due to conflicting blocks.
More precisely, let $e_1, e_2, e_3, e_4$ be events
and $B, B'$ be blocks such that $B \neq B'$, $\VariableOf{B} = \VariableOf{B'}$
$e_2, e_3 \in B$ and $e_4 \in B'$.
If $e_1 \bhbseq e_2$ and $e_3 \bhbseq e_4$,
then for every event $e_5 \in \after{\bhbseq}(B') = \bigcup\limits_{e \in B'} \after{\bhbseq}(e)$,
we must have $e_1 \bhbseq e_5$.
% Here, by $\after{\bhbseq}(B')$ we mean
% the set $\bigcup\limits_{e \in B'} \after{\bhbseq}(e)$.
In order to track dependencies of the latter kind in constant space,
our algorithm will track auxiliary data that will reflect the following collection of $\bhbseq$-after sets.
\begin{align}
\begin{array}{rcl}
\blkafter{\bhbeq}(e) &=& \setpred{\after{\bhbseq}(B)}{B \in \blocks, \exists i \in B, e \bhbseq i} \\
\end{array}
\end{align}
Observe that, even though, for a given block $B$, $\after{\bhbseq}(B)$
has constant size, the number of such blocks $B$ for which
$e \bhbseq i$ for some $i \in B$ may be unbounded.
This is one of the key challenges in the design of a constant space algorithm for tracking
an inductive partial order such as $\bhbseq$.
Fortunately, the following observation comes to rescue.
\begin{proposition}
\proplabel{fst-block}
% Let $\extendBlk{\tr} \in \extendBlk{\alphabet}^*_\noval$ be an annotated execution corresponding to $\tr \in \alphabet^*_\noval$ and blocks $\blocks$.
Let $x \in \vars$ and let $t \in \threads$.
Let $e$ be an event
and let 
% $S_{t, x, e} = \setpred{B \in \blocks}{\VariableOf{B} = x, \ThreadOf{B} = t \text{ and } \exists i \in B, e \bhbseq i}$, 
$S_{t, x, e}$ be the collection of all
blocks $B$ such that $\VariableOf{B} = x, \ThreadOf{B} = t$
and $\exists f \in B, e \bhbseq f$.
Here we use the shorthand $\ThreadOf{B}$ to denote
$\ThreadOf{e^\wt_B}$, where $e^\wt_B$ is the unique write event in $B$.
Let $B_{\sf fst}$ be the first block in $S_{t, x, e}$.
Then, for every block $B' \in S_{t, x, e} \setminus \set{B_{\sf fst}}$
and for every event $f \in B'$, we must have
$e \bhbseq f$.
\end{proposition}
In other words, \propref{fst-block} ensures that instead of keeping track of all
blocks that are $\bhbseq$ after a given event $e$,
it suffices to only track one (namely the first) relevant block per thread and variable.
Armed with this insight, we define the following.
\begin{align}
\begin{array}{rcll}
\fstblkafter{\bhbeq}{t}{x}(e) &=& \setpred{\after{\bhbseq}(B)}{&B \in \blocks \text{ is the first block such that } \\ &&& \VariableOf{B} = x, \ThreadOf{B} = t, \exists f \in B, e \bhbseq f} \\
\end{array}
\end{align}
Here, as in \propref{fst-block}, the shorthand $\ThreadOf{B}$ denotes
$\ThreadOf{e^\wt_B}$, where $e^\wt_B$ is the unique write event in $B$.
The advantage of the above definition can be
formalized as follows.
\begin{proposition}
\proplabel{fst-block-one}
% Let $\extendBlk{\tr} \in \extendBlk{\alphabet}^*_\noval$ be an annotated execution corresponding to $\tr \in \alphabet^*_\noval$ and blocks $\blocks$.
Let $e$ be an event.
For every set $S \in \blkafter{\bhbeq}(e)$, there is a thread $t$, variable $x$ 
and a set $S' \in \fstblkafter{\bhbeq}{t}{x}(e)$ such that $S \subseteq S'$.
\end{proposition}
}

\myparagraph{Fine State Automaton}{
We now have most of the ingredients for
our algorithm that tracks $\bhbs$ (more precisely $\bhbseq$)
and now proceed to 
present our constant-space algorithm
as a deterministic finite state automaton.
The automaton processes an input word $\extendBlk{\tr}$ over $\extendBlk{\alphabet}_\noval$,
one symbol at a time.
Recall that the choice of blocks is ingrained into the word
using the annotations $\set{\tru, \fls}$.
The states of the automaton track the saturated partial order
$\bhbseq$ induced by the input word's annotations
by maintaining, for  every letter $a \in \extendBlk{\alphabet}_\noval$,
the set $\after{\bhbseq}(e_a)$ where $e_a$ is the last event
seen in the word such that $\extendBlk{\tr}[e_a] = a$.
The precise definition of the automaton is presented next,
and the precise invariant maintained by it is presented in
\thmref{automata-saturation-invariant}.
The components of our \underline{sat}uration automaton are
\[\autsup{\saturated} = (\statessup{\saturated}, \initsup{\saturated}, \transsup{\saturated})\]
where $\statessup{\saturated}$ is the set of states,
$\initsup{\saturated} \in \statessup{\saturated}$ is a dedicated initial state
and $\transsup{\saturated} : \statessup{\saturated} \times \extendBlk{\alphabet}_\noval \to \statessup{\saturated}$
is the transition function. 
We next describe the crucial insights behind the automaton construction. 
For brevity, some technical details are postponed to \appref{app-automata}.
}

\myparagraph{\it \underline{States of $\autsup{\saturated}$}}{
	Each state $q \in \statessup{\saturated}$ is a tuple of the form
	\[
		q = (\autBlks, \autRF, \autAfterSat, \autBlkAfter, \autBlkAfterOpen)
	\]
	where,
	\begin{itemize}
		\item $\autBlks : \vars \partialto \powset{\extendBlk{\alphabet}_\noval}$
		maps each variable $x \in \vars$ to the contents of the running block $B_x$ on variable $x$
		in the concurrent program run seen so far. If no such block exists, $\autBlks(x) = \emptyset$,

		\item $\autRF : \vars \partialto \extendBlk{\alphabet}_\noval$ maps each variable $x$
		to the label of the last write on $x$. This will be used to track the reads-from dependency
		for read events,

		\item $\autAfterSat : \extendBlk{\alphabet}_\noval \to \powset{\extendBlk{\alphabet}_\noval}$
		maps each symbol $a \in \extendBlk{\alphabet}_\noval$ to the after set $\after{\bhbseq}(e_a)$
		induced by the saturated order $\bhbseq$,
		where $e_a$ is the last event with label $a$,

		\item The map $\autBlkAfter : \extendBlk{\alphabet}_\noval \times \threads \times \vars \to \powset{\extendBlk{\alphabet}_\noval}$ is such that,
		for each symbol $a \in \extendBlk{\alphabet}_\noval$,
		thread $t$ and variable $x$, $\autBlkAfter(a, t, x)$
		stores the $\bhbseq$-after set of the first block $B_{t,x}$ such that
		$\ThreadOf{B} = t$, $\VariableOf{B} = x$, and
		there is an event $e \in B_{t,x}$ such that $e_a \bhbseq e$;
		here, $e_a$ is the latest event with label $a$.
		
		\item Finally, $\autBlkAfterOpen : \extendBlk{\alphabet}_\noval \times \threads \times \vars \to \set{\tru, \fls}$ is such that $\autBlkAfterOpen(a, t, x)$  
		tracks if the block $B_{t,x}$ defined above is currently open.
	\end{itemize}
	The components of a given state $q$ will be refered to as $q.\autBlks$, $q.\autRF$, $q.\autAfterSat$ and $q.\autBlkAfter$.
}

\myparagraph{\it \underline{Initial State of $\autsup{\saturated}$}}{
	The initial state $\initsup{\saturated} \in \statessup{\saturated}$
	is such that
	$\autRF(x) = \undf$,
	 $\autBlks(x) =  \autAfterSat(a) = \autBlkAfter(a,t,x) = \emptyset$,
	and, $\autBlkAfterOpen(a, t,x) = \top$ for each $a \in \extendBlk{\alphabet}_\noval$, $t \in \threads$ and $x \in \vars$.
}

\myparagraph{\it \underline{Transitions of $\autsup{\saturated}$}}{
	The transitions of the automaton are detailed, but intuitive.
	For a given $q \in \statessup{\saturated}$ and symbol $a \in \extendBlk{\alphabet}_\noval$,
	let $q' = \transsup{\saturated}(q, a)$ be the resulting state.
	The components $q'.\autBlks$, $q'.\autRF$ and $q'.\autBlkAfterOpen$ are straightforward.
	We discuss here the more subtle components $q'.\autAfterSat$ and $q'.\autBlkAfter$.
	Again, precise definitions can be found in \appref{app-automata}.

	Let us see how the components $\autAfterSat$ and $\autBlkAfter$ get updated
	and understand why the updates are involved.
	Suppose there is a symbol $c$ such that the input symbol $a$
	on the transition induces a $\bhbeq$ dependency 
	with some $a' \in \autAfterSat(c)$.
	Then, $a$ should be added to $\autAfterSat(c)$ since we would inductively have $e_c \bhbseq e_1$,
	where $e_c$ denotes some prior event labeled with the symbol $c$, and $e_a$
	denotes the new event labeled with $a$.
	This, in turn, mean that $a'$ should also be added to
	$\autBlkAfter(c', t, x)$ if it contains $c$.
	More importantly, if the first block $B_{t,x}$ $\bhbseq$-after $c'$
	is closed and $\VariableOf{a} = x$, then $a$ must also be
	added to $\autAfterSat(c')$.
	This chain of reasoning can continue even further.
	In view of this, we present a least fixpoint style
	formulation for the new maps $q'.\autAfterSat$ and $q'.\autBlkAfter$.

	We define sets $\setpred{A_c}{c \in \extendBlk{\alphabet}_\noval}$ and 
	$\setpred{FBA_{c, t, x}}{c \in \extendBlk{\alphabet}_\noval, t \in \threads, x \in \vars}$ as the smallest
	sets that satisfy the following conditions:
	\begin{align*}
	\begin{array}{rl}
		\deprf(a) \cap A_c \implies a \in A_c & \text{ for every } c \\[0.5em]
		q.\autAfterSat(c) \subseteq A_c & \text{ for every } c \\[0.5em]
		q.\autBlkAfter(c, t, x) \subseteq FBA_{c, t, x} & \text{ for every } c, t, x \\[0.5em]
		\deprf(d) \cap A_c \implies A_d \subseteq A_c & \text{ for every } c, d \\[0.5em]
		\deprf(d) \cap FBA_{c, t, x} \implies A_d \subseteq FBA_{c, t, x} & \text{ for every } c, t, x, d \\[0.5em]
		\!\!\!\begin{array}{l}
		d \in A_c %\\
		\land \, q.\autBlkAfter(c, t, x) = \emptyset %\\
		\end{array}\!\!
		{\implies} 
		A_{d'} \subseteq FBA_{c, t, x} 
		&\!\!\!\begin{array}{l}
		\text{ for every } c, d, d', t, x, \text{ with } t = \ThreadOf{d}, \\
		\,x = \VariableOf{d}, 
		\AnnotOf{d} = \top, d' \in q'.\autBlks(x)
		\end{array} \\[1em]
		\!\!\!\begin{array}{c}
		d \in FBA_{c, t, x} %\\
		\land \, q.\autBlkAfterOpen(c, t, x) = \bot 
		\end{array}\!\!
		{\implies} 
		A_d \subseteq A_c
		&\!\!\!\begin{array}{l}
		\text{ for every } c, d, t, x \text{ with } t = \ThreadOf{d}, \\
		\,x = \VariableOf{d}, \AnnotOf{d} = \top
		\end{array}
	\end{array}
	\end{align*}
	Here, for a symbol $c \in \extendBlk{\alphabet}_\noval$,
	we use the notation: 
	\begin{align*}
	\begin{array}{lcr}
	\deprf(c) &=& 
	\begin{cases}
		\setpred{c'}{(c, c') \in \annotDep} & \text{ if } \OpOf{c} = \wt \\
		\setpred{c'}{\set{(c, c'), (c_{\rdf{}}, c')} \cap \annotDep \neq \emptyset} & \text{ otherwise if } \OpOf{c} = \rd \text{ and } c_{\rdf{}} = q.\autRF(\VariableOf{c})
	\end{cases} \\
	\text{where, }
	\annotDep &=& \deprel_\noval \times \set{\top, \bot} \setminus \setpred{(a, b)}{\ThreadOf{a} \neq \ThreadOf{b} \text{ and } \AnnotOf{a} = \AnnotOf{b} = \top}
	\end{array}
	\end{align*}
	We remark that the sets $\setpred{A_c}{c \in \extendBlk{\alphabet}_\noval}$
	and $\setpred{FBA_{c,t,x}}{c \in \extendBlk{\alphabet}_\noval, t\in\threads, x \in\vars}$ can be computed in an iterative manner
	in time that is linear in 
	the size of a state $O(|\extendBlk{\alphabet}_\noval|{\cdot}|\threads|{\cdot}|\vars|)$ 
	which is a constant.

	Having defined these fixpoint sets, we can now define $q'.\autAfterSat$ and $q'.\autBlkAfter$ as follows. 
	First, $q'.\autAfterSat(a) = \set{a}$, and for every other $c \neq a$,
	$q'.\autAfterSat(c) = A_c$.

	Next, the sets $q'.\autBlkAfter$ are described as follows.
	For the input letter $a$,
	$q'.\autBlkAfter(a, t, x)$ is $\set{a}$ if $a$ corresponds to a write event on $x$ in thread $t$
	that starts a new block,
	is $A_{a_{\rdf{}}}$ if $a$ corresponds to a read event of $x$ in thread $t$, 
	and $\emptyset$ otherwise.
	For every other symbol $c \neq a \in \extendBlk{\alphabet}_\noval$, $q'.\autBlkAfter(c, t, x) = FBA_{c, t, x}$.
}



This concludes an informal description of the automaton $\autsup{\saturated}$ (see \appref{app-automata} for full details).
We state the key invariant useful for designing later algorithms in \thmref{automata-saturation-invariant}.
A stronger, more detailed, invariant helpful in establishing \thmref{automata-saturation-invariant}
can be found in \appref{app-automata}.

\begin{theorem}
\thmlabel{automata-saturation-invariant}
Let $\tr \in \alphabet_\noval^+$, $\blocks$ be a set of blocks in $\tr$
and let $\extendBlk{\tr} \in \extendBlk{\alphabet}_\noval^*$ be the corresponding annotated program run.
Let $q = \transsup{\saturated}^*(\initsup{\saturated}, \extendBlk{\tr})$
be the state reached by the automaton $\autsup{\saturated}$ on the string $\extendBlk{\tr}$.
For a symbol $a \in \extendBlk{\alphabet}_\noval$, let $e_a$ be the last event in 
$\extendBlk{\tr}$ such that $\extendBlk{\tr}[e_a] = a$.
Then we have that, for every $a \in \extendBlk{\alphabet}_\noval$,
		$q.\autAfterSat(a) = \after{\bhbseq}(e_a)$ if $e_a$ exists; and $\emptyset$ otherwise.
\end{theorem}

==> block-partial-order.tex <==
% !TEX root = main.tex

\section{Block Partial Order}\label{sec:bpo}


==> block-selection.tex <==
%!TEX root=./main.tex

\subsection{Selection of Blocks}
\seclabel{select-blocks}

So far, the notion of commutativity and the corresponding notion
of equivalence $\fbeq$ we have been working with, is parametric
in the choice of block $\blocks$.
This means, for checking a property on a concurrent execution,
one additionally needs to decide which events participate in blocks and which others do not.
In the context of determining a property such as causal concurrency,
a sub-optimal choice of blocks may deem two events causally ordered,
even though a more optimal choice may deem them concurrent.
Can we find the best choice of blocks?
In this section, we answer this question in the positive,
by generalizing 
the notion of equivalence discussed so far so that it
does retain the expressive power of block swaps, yet does not 
rely on explicitly providing the choice of blocks.
Our solution is to resort to \emph{all} choices of block selections.
Towards this, we deem two executions equivalent under our new, more general, notion of equivalence,
if they can be deemed equivalent under $\fbeq$ for any choice of $\blocks$.
We formalize this next.

\begin{definition}[\orclFreeBlkText Equivalence $\ofbeq$]
\deflabel{oracle-free-beq}
Let $w \in \alphabet_\noval^*$ and let $\libAtBlks$
be the collection of sets of blocks $\blocks$ each of which is
liberally atomic.
% $\libAtBlks = \setpred{\blocks}{\blocks \text{ is a valid \\ set of liberally atomic blocks of } w}$.
For a string $w' \in \alphabet_\noval^*$, we say that
$w \ofbeq w'$ if there is a set $\blocks \in \libAtBlks$ such that
$w \fbeq w'$.
\end{definition}

% \ucomment{Give examples}

\myparagraph{Concurrency Up to \orclFreeBlkText Equivalence}{
	We now consider the problem of determining causal concurrency
	under the new notion $\ofbeq$ --- given symbols $c$ and $d$
	and input run $\tr\in \alphabet_\noval^*$, check if $\checkConcSymb{\ofbeq}{\tr}{c}{d}$ holds.
	This is achieved using a guess-and-check framework.
	That is, given $\tr$, we guess the set of blocks $\blocks$ of $\tr$
	and check if $\checkConcSymb{\fbeq}{\extendBlk{\tr}}{c}{d}$ holds.

	Let us fix some notation here.
	For a string $w' \in \extendBlk{\alphabet}_\noval^*$, we use
	$\unannot{w'}$ to be the string $w \in \alphabet_\noval^*$
	obtained by projecting $w'$ onto the alphabet $\alphabet_\noval$.
	Let us say that an annotated string $w' \in \extendBlk{\alphabet}_\noval^*$
	is \emph{well-annotated} if the annotations used in $w'$ are consistent with block boundaries
	in $w = \unannot{w'}$.
	% Let $w \in \alphabet^*_\noval$ be the string obtained by projecting out
	% the annotations.
	That is, $w'$ is well-annotated if for every read event $e = \ev{t, \rd, x} \in \events{w}$
	with writer event $e_{\rdf{}} = \rdf{w}(e)$,
	we have
	$\AnnotOf{w'[e]} = \top$ iff $\AnnotOf{w'[f]} = \top$ for every $f$ that
	is either $e_{\rdf{}}$ or a read event that reads from  $e_{\rdf{}}$.
	 % \in \set{e_{\rdf{}}} \setpred{g}{\rdf{g} = e_{\rdf{}}}$.
	Let $L_\textsf{well-annotated} = \setpred{\tr' \in \extendBlk{\alphabet}_\noval^*}{\tr' \text{ is valid}}$.
	It is to see that $L_\textsf{well-annotated}$ is a regular language.
	
	Recall from \secref{cc-alg} that $L_{c, d}$ is the set of strings accepted by
	the automaton $\autsup{c, d}$ that simultaneously checks liberal atomicity 
	and concurrency between occurrences of symbols $c$ and $d$ in an annotated word.
	Now consider the language $L_\textsf{well-annotated, c, d} = L_\textsf{well-annotated} \cap L_{c, d}$.
	Consider an annotated run $\tr' \in \extendBlk{\alphabet}_\noval^*$.
	If $\tr' \in L_\textsf{well-annotated, c, d}$, then we must have 
	$\checkConcSymb{\ofbeq}{\tr}{c}{d}$, where $w = \unannot{w}$.
	Since regular languages are closed under intersection, we have that 
	$L_\textsf{well-annotated, c, d}$ is regular and thus the problem of checking ---
	if an annotated string is well-annotated with liberally atomic blocks
	and renders tw occurences of $c$ and $d$ concurrent --- can be solved using a constant space algorithm.

	Now, consider the following language: 
	\[
	L_{c, d, \mathsf{deannot}}  = \setpred{\tr \in \alphabet^*_\noval}{\exists \tr' \in L_\textsf{well-annotated, c, d}, \tr = \unannot{\tr'}}
	\]
	Since $L_\textsf{well-annotated, c, d}$ is regular, and since
	regular languages are closed under
	projection, we have that $L_{c, d, \mathsf{deannot}}$ is regular.
	Finally, it is easy to also observe that the following equality holds:
	\[
	L_{c, d, \mathsf{deannot}}  = \setpred{\tr \in \alphabet^*_\noval}{\checkConcSymb{\ofbeq}{\tr}{c}{d}}
	\]
	This gives us the following result.

	\begin{theorem}
	The problem of checking causal concurrency under $\ofbeq$ is solvable using a one pass streaming algorithm that runs in constant space.
	\end{theorem}
}

==> cc-block-algo.tex <==
%!TEX root = ./main.tex

\subsection{Checking Causal Concurrency}
\seclabel{cc-alg}

Let us now get back to the problem of checking
causal concurrency up to the equivalence induced by a given set of liberally atomic blocks.
More precisely, in this section  we want to design 
a constant space algorithm for solving \probref{cc-symb}.
In particular, for each pair of symbols $\extendBlk{c}, \extendBlk{d} \in \extendBlk{\alphabet}_\noval$,
we construct an automaton $\autsup{\extendBlk{c},\extendBlk{d}}$,
such that, for every run $\tr$ and blocks $\blocks$, 
the corresponding
annotation $\extendBlk{\tr}$ 
is accepted by $\autsup{\extendBlk{c},\extendBlk{d}}$ iff $\checkConcSymb{\fbeq}{\extendBlk{\tr}}{\extendBlk{c}}{\extendBlk{d}}$.
Observe that, for a given pair $c, d \in \alphabet_\noval$,
determining if $\checkConcSymb{\fbeq}{\tr}{c}{d}$ amounts to checking
if there is some $(\extendBlk{c}, \extendBlk{d}) \in \setpred{\big((c, \alpha), (c, \beta)\big)}{\alpha, \beta \in \set{\top, \bot}}$ for which $\checkConcSymb{\fbeq}{\extendBlk{\tr}}{\extendBlk{c}}{\extendBlk{d}}$.

Our first observation is that $\fbeq$ preserves $\po{}$ and thus
it suffices to check only the \emph{inner} occurrences of $\extendBlk{c}$
and $\extendBlk{d}$.
Two events $e$ and $f$ are said to be inner occurences of $\extendBlk{c}$
and $\extendBlk{d}$
if $\extendBlk{\tr}[e] = \extendBlk{c}$, $\extendBlk{\tr}[f] = \extendBlk{d}$,
$e$ occurs before $f$ in $\tr$
and $f$ is the first such event after $e$.
Towards this, the automaton $\autsup{\extendBlk{c},\extendBlk{d}}$
can be constructed by directly extending $\autsup{\libat}$ as follows.
Each state of $\autsup{\extendBlk{c},\extendBlk{d}}$ is a tuple
$q = (q_\libat, C, \mathsf{b})$ where $q_\libat$ is a state of
the liberal atomicity checking automaton $\autsup{\libat}$,
$C \subseteq \extendBlk{\alphabet}_\noval$ stores the set $\after{\bhbseq}(e_c)$,
where $e_c$ is the last event of label $\extendBlk{c}$, and $\mathsf{b} \in \set{\top, \bot}$ tracks if, so far in the input program run,
we have found an event pair $(e, f)$ that witnesses $\checkConcSymb{\fbeq}{\extendBlk{\tr}}{\extendBlk{c}}{\extendBlk{d}}$.
The transitions are intuitive and we skip the details.
The set of final states are those $(q, \mathsf{b})$ such that $q \in \finalsup{\libat}$ and $\mathsf{b} = \top$.
Let $L_{c,d} = \bigcup\limits_{\alpha, \beta \in \set{\top, \bot}} L(\autsup{(c, \alpha), (d, \beta)})$.
Observe that $L_{c, d}$ defined this way is a regular language.
Let us fix $\autsup{c, d}$ to be some deterministic finite state automaton
with $L(\autsup{c, d}) = L_{c, d}$.
$\autsup{c, d}$ is then our desired constant space algorithm.
\begin{theorem}
Given $c, d \in \alphabet_\noval$, run $\tr$, blocks $\blocks$, the predicate
$\checkConcSymb{\fbeq}{\tr}{c}{d}$ can be determined using a one pass streaming
algorithm that processes the corresponding annotated run $\extendBlk{\tr}$ 
using constant space.
\end{theorem}

==> check-order.tex <==
% !TEX root = main.tex

\subsection{Causal Ordering and Causal Concurrency}
\seclabel{check-order-semantic}

In scenarios like dynamic partial order reduction in stateless model checking,
or runtime predictive monitoring, one is often interested in
the \emph{causal relationship} between actions.
Understanding causality at the level of program runs often amounts to
answering whether there is an equivalent run that witnesses
the inversion of order between two  events.

\myparagraph{Ordering and Concurrency}{
Formally, let $\sim$ be an equivalence over $\alphabet^*$ such that when two runs
are $\sim$~equivalent, they are also permutations of each other.
Let $w \in \alphabet^*$ be a concurrent program run, and let $e, f \in \events{w}$ 
be two events occurring at indices $i$ and $j$ (with $i < j$).
We say that $e$ and $f$ are \emph{causally ordered} in $w$
if for every equivalent string $w' \sim w$,
the corresponding indices $i'$ and $j'$ where respectively $e$ and $f$ occur in $w'$
are such that $i' < j'$.
We use $\checkOrder{\sim}{w}{e}{f}$ to denote that
events $e$ and $f$ are causally ordered in $w$.
If $e$ and $f$ are not causally ordered under an equivalence $\sim$,
we say that they are causally concurrent under $\sim$,
and denote this using $\checkConc{\sim}{w}{e}{f}$.
}

The following are the key algorithmic questions we investigate in this paper.
Recall that we only consider equivalence relations that deem two runs equivalent
only when they are permutations of each other.
\begin{problem}[Checking Causal Concurrency Between Events]
\problabel{conc-events}
Let $\sim$ be an equivalence over $\alphabet^*$.
Given an execution $w \in \alphabet^*$, and two events
$e, f \in \events{w}$, the problem of checking causal concurrency between events 
asks to determine if $\checkOrder{\sim}{w}{e}{f}$.
\end{problem}
% \begin{problem}[Checking Causal Concurrency]
% Let $\sim$ be an equivalence over $\alphabet^*$.
% Given an execution $w \in \alphabet^*$, and two events
% $e, f \in \alphabet$, the causal 
% concurrency problem asks to determine if there are events
% labelled $c$ and $d$ that are causally concurrent,
% i.e., if there are indices $i, j \in \range{|w|}$ such that
% $i < j$, $w[i] = c, w[j] = d$, we have $\checkOrder{\sim}{w}{i}{j}$.
% We denote this using $\checkConc{\sim}{w}{c}{d}$
% \end{problem}

In the context of many applications in testing and verification
of concurrent programs, one often asks a slightly more coarse grained question,
which we state below.
\begin{problem}[Checking Causal Concurrency Between Symbols]
\problabel{cc-symb}
Let $\sim$ be an equivalence over $\alphabet^*$.
Given an execution $w \in \alphabet^*$, and two labels
or letters $c, d \in \alphabet$, 
the problem of checking causal concurrency between symbols (or letters)  
asks to determine if 
there are events $e, f \in \events{w}$ such that $w[e] = c$, $w[f] = d$
and $\checkConc{\sim}{w}{e}{f}$.
We denote this with $\checkConcSymb{\sim}{w}{c}{d}$.
\end{problem}

\begin{remark}
The predicate $\checkConcSymb{\sim}{w}{c}{d}$ can be used to answer the more fine-grained question of determining
whether two given events $e$ and $f$ are causally concurrent (i.e., $\checkConc{\sim}{w}{e}{f}$) or ordered.
In particular, we take $c = w[e]$ and $d = w[f]$,
and consider the alphabet $\Delta = \alphabet \uplus \set{c^{\focalEv}, d^{\focalEv}}$,
where $c^{\focalEv_1}$ and $d^{\focalEv_2}$ are distinct marked copies of the letters $c, d \in \alphabet$.
Consider the string $w' \in \Delta^*$ with $|w'| = |w|$
such that $w'[g] = w[g]$ for every $g \not\in \set{e, f}$,
$w[e] = c^{\focalEv_1}$ and $w[f] = d^{\focalEv_2}$.
Then, $\checkConcSymb{\sim'}{w'}{c^{\focalEv_1}}{d^{\focalEv_2}}$ holds iff $\checkConc{\sim}{w}{e}{f}$, where
the equivalence $\sim'$ is the same as $\sim$, modulo renaming letters $c^{\focalEv_1}$ and $d^{\focalEv_2}$
to $c$ and $d$ respectively.
\end{remark}

\subsection{Computational Hardness in Checking Concurrency}

The efficiency of determining the answer to $\checkConc{\sim}{w}{c}{d}$
is key in designing efficient techniques, for, say, dynamic 
detection of concurrency bugs such as data races, deadlocks, or violations of atomicity.
When deploying such techniques for monitoring 
large scale software
artifacts exhibiting executions with billions of events,
a desirable goal is to design monitoring algorithms that 
can be efficiently implemented in an online `incremental' fashion
that store only a constant amount of information, independent of 
the size of the execution being monitored~\cite{RV03RTA}, which can otherwise
grow arbitrarily large.
In other words, an ideal algorithm would observe events in an execution
in a single forward pass, using a small amount of memory.
This motivates our investigation of the efficiency of checking causal ordering.

Indeed, for the case of trace equivalence,
causal concurrency can be determined in a constant space
streaming fashion.

\begin{lemma}[Causal concurrency for trace equivalence]
Given an input $w \in \alphabet^*$ and symbols $c, d \in \alphabet$,
the predicate
$\checkConcSymb{\mazeq{}}{w}{c}{d}$ can be determined using a single pass constant space
streaming algorithm.
\end{lemma}

% In \secref{gmonitor}
The above follows from the observation that if two events $e$ and $f$
(labeled with, respectively $c$ and $d$) in $w$ are causally ordered
according to $\mazeq{}$, then there is a sequence of events
$e = g_1, \ldots, g_n = f$ that occurs between
$e$ and $f$, such that $(w[g_{i}], w[g_{i+1}]) \in \deprel$ for every $i < n$.
This observation can be used to design a constant space
monitoring algorithm for checking $\checkConcSymb{\mazeq{}}{w}{c}{d}$;
we present it in greater detail in \secref{gmonitor}.
% This means that $w$ must not belong to any of the regular languages
% $L_a = \alphabet^* \,c\, \alphabet^* \, a \, \alphabet^* \, d \, \alphabet^*$,
% where $\set{(a,c), (a, d)} \subseteq \deprel$.
% This corresponds to a membership question for regular languages, solvable in constant space
% using their corresponding finite automata.

In this section, we show that the above desirable goal, 
however, is not achievable for the case of reads-from equivalence --- we show that any algorithm
for checking causal ordering (for the semantic notion of equivalence $\rfnovaleq$)
must use linear space in a streaming setting.
\begin{theorem}[Linear space hardness]
\thmlabel{check-order-semantic-linear-space-lower-bound}
Any streaming algorithm that determines the predicate $\checkConcSymb{\rfnovaleq}{\cdot}{\cdot}{\cdot}$
in a streaming fashion uses linear space, even for inputs runs containing
just $2$ threads and $6$ variables.
\end{theorem}

The key idea behind the proof of \thmref{check-order-semantic-linear-space-lower-bound}
is to exploit and generalize the intricate pattern in the runs in \figref{intro}.
In essence, the pattern is such that the question of causal concurrency,
between two specific events in the pattern, requires us to successively infer the concurrency status
of linearly many pairs of events, placed arbitrarily far away in the past and/or in the future,
which is impossible for a one pass streaming algorithm
that only uses sub-linear space.
The formal proof, inspired  inspired from similar results in the context of data race prediction~\cite{Kini17,Mathur21} is presented in~\appref{hardness}
and constructs a constant space, one pass, linear time reduction from the following language
language, parametrized by $n \in \natsp$, which admits a linear space lowerbound for its membership question:
\begin{align*}
\langeq_n = \setpred{\vect{a}\#\vect{b}}{\vect{a}, \vect{b} \in \set{0,1}^n \text{ and } \vect{a} = \vect{b}}
\end{align*}

In fact, we use similar ideas as above to also establish a lower bound on the time-space tradeoff for
the problem of determining causal concurrency, even when we do not bound the number of passes;
formal proof is deferred to \appref{hardness}:
\begin{theorem}[Quadratic time space lower bound]
\thmlabel{check-order-semantic-tradeoff}
For any algorithm (streaming or not) that determines the predicate 
$\checkConcSymb{\rfnovaleq}{\cdot}{\cdot}{\cdot}$ in $S(n)$ space and $T(n)$ time
on input runs of length $n$, we must have $S(n) \cdot T(n) \in \Omega(n^2)$.
\end{theorem}

% The proofs of both \thmref{check-order-semantic-linear-space-lower-bound}
%  and \thmref{check-order-semantic-tradeoff}
% are established using a
%  constant space streaming reduction to the following language,
%  parametrized by $n$, which also
%  admits a linear space lower bound for the membership problem. 
% \begin{align*}
% \langeq_n = \setpred{\vect{a}\#\vect{b}}{\vect{a}, \vect{b} \in \set{0,1}^n \text{ and } \vect{a} = \vect{b}}
% \end{align*}
% The proofs are relegated to \appref{hardness}.
% The insight used behind the reduction is inspired by the runs in \figref{intro} --- determining
% whether two events can be reordered depends upon arbitrarily far away events in the past and/or the future, making it difficult to track ordering constraints when limited to sub-linear space.
% We present the proof next.
% Our reductions are inspired from similar results in the context of data race prediction~\cite{Kini17,Mathur21}.


Next we show that the problem of determining concurrency
is also not context-free. 
% \begin{theorem}[Non Context-freeness]
% \thmlabel{check-order-non-context-free}
% Let $c, d \in \alphabet$.
% There is no non-deterministic push-down automaton that recognizes the following set of words:
% \[
% L^{c,d}_{\textsf{ordered}} = \setpred{\tr \in \alphabet^*}{\neg \checkConcSymb{\rfnovaleq}{\tr}{c}{d} }
% \]
% \end{theorem}

\begin{theorem}[Non Context-freeness]
\thmlabel{check-order-non-context-free}
% The problem of checking if for a given run $\tr$ and two symbols $c, d$
Let $c, d \in \alphabet$.
There is no nondeterministic pushdown automaton that accepts exactly the
runs $\tr$ such that both $c$  and $d$ appear in $\tr$
but $\checkConcSymb{\rfnovaleq}{\tr}{c}{d}$.
% \[
% L^{c,d}_{\textsf{ordered}} = \setpred{\tr \in \alphabet^*}{\neg \checkConcSymb{\rfnovaleq}{\tr}{c}{d} }
% \]
\end{theorem}

Finally, we show that the problems of checking $\checkConcSymb{\rfnovaleq}{\cdot}{\cdot}{\cdot}$ and $\checkConc{\rfnovaleq}{\cdot}{\cdot}{\cdot}$ both admit a quadratic time lower bound, conditioned on 
the widely believed Strong Exponential Time Hypothesis (SETH)~\cite{ImpagliazzoP01}.


\begin{theorem}
\thmlabel{quadratic-time-hardness}
Assume SETH. The problem of determining $\checkConc{\rfnovaleq}{\tr}{e}{f}$ cannot be solved in time $O(|\tr|^{2-\epsilon})$ for all $\epsilon>0$, even when $\tr$ has $2$ threads ($e, f$ are events in $\tr$).
\end{theorem}

The formal proof of \thmref{quadratic-time-hardness} is presented in \appref{ov-hardness}. 
It is established via a fine-grained reduction from the Orthogonal Vector Conjecture,
which also admits a quadratic lower bound under (SETH)~\cite{Williams05}.
The input to the Orthogonal Vectors (OV) problem is a pair of sequences $A, B \subseteq \set{0,1}^d$ of $d$-dimensional vectors, each of length $n$ (i.e., $|A| = |B| = n$), and the output is YES iff
there is are two vectors $a \in A, b \in B$ such that their inner product is $0$ (i.e., $a \cdot b = 0$). 
The OV hypothesis states that for every $\epsilon > 0$, 
there is no algorithm that solves the OV problem 
(with input instances of length $n$ and dimension $d$, with $d = \Omega(\log n)$) in $O(n^{2-\epsilon}\poly(d))$.


\begin{comment}
\ucomment{Give examples explaining the intuition behind non-triviality involved in answering this question.}

Before we present the formal proof, let us discuss some examples to understand
some basic intuitions behind the source of hardness.

\begin{example}
\ucomment{Example to show that po and rf dependencies must be respected. Follows easily
from def. Then formulate a proposition out of it.}
\end{example}

\begin{example}
\ucomment{Example to show dependencies can be recursive. Explain the implication --- events way in the past can affect the decision. Same for events in the future. State proposition stating implied dependencies.}
\end{example}


\begin{lemma}
\lemlabel{properties-check-order-semantic}
Let $w \in \alphabet^*$ be an execution.
The relation $\ctrf{w} = \setpred{(i, j)}{i, j \in \range{|w|}, \checkOrder{\rfnovaleq}{w}{i}{j}}$
satisfies the following properties:
% \begin{enumerate}[label=(\arabic*)]
% 	% \item $\ctrf{w}$ is consistent with the total order induced by $w$. 
% 	% That is, for every $i \neq j  \in \range{|w|}$, if $i \ctrf{w} j$, then $i < j$.
% 	\item $\ctrf{w}$ is a partial order. That is, $\ctrf{w}$ is irreflexive and transitive.
% 	\item $\ctrf{w}$ orders events of $w$ in the same thread. 
% 	That is, for every $i < j \in \range{|w|}$, if
% 	$\ThreadOf{w[i]} = \ThreadOf{w[j]}$, then $i \ctrf{w} j$.
% 	\item $\ctrf{w}w$ orders events if there is a reads-from dependency between them.
% 	That is, for every $i < j \in \range{|w|}$, if $\rdf{w}(j) = i$, then $i \ctrf{w} j$.
% 	\item Let $i, j, k \in \range{|w|}$ be distinct indices such that
% 	such that $\VariableOf{i} = \VariableOf{j} = \VariableOf{k}$,
% 	$\OpOf{i} = \OpOf{k} = \wt$ and $\OpOf{j} = \rd$
% 	and $\rdf{w}(j) = i$.
% 	\begin{enumerate}[label=(4.\alph*)]
% 		\item If $i \ctrf{w} k$, then $j \ctrf{w} k$.
% 		\item If $k \ctrf{w} j$, then $k \ctrf{w} i$.
% 	\end{enumerate}
% \end{enumerate}
\begin{description}
	% \item $\ctrf{w}$ is consistent with the total order induced by $w$. 
	% That is, for every $i \neq j  \in \range{|w|}$, if $i \ctrf{w} j$, then $i < j$.
	\item[(Partial order).] $\ctrf{w}$ is a partial order. That is, $\ctrf{w}$ is irreflexive and transitive.
	\item[(Intra-thread order).] $\ctrf{w}$ orders events of $w$ in the same thread. 
	That is, for every $i < j \in \range{|w|}$, if
	$\ThreadOf{w[i]} = \ThreadOf{w[j]}$, then $i \ctrf{w} j$.
	\item[(Reads-from).] $\ctrf{w}w$ orders events if there is a reads-from dependency between them.
	That is, for every $i < j \in \range{|w|}$, if $\rdf{w}(j) = i$, then $i \ctrf{w} j$.
	\item[(Implied orders).] 
	\itmlabel{implied-order-semantic}
	Let $i, j, k \in \range{|w|}$ be distinct indices such that
	such that $\VariableOf{i} = \VariableOf{j} = \VariableOf{k}$,
	$\OpOf{i} = \OpOf{k} = \wt$ and $\OpOf{j} = \rd$
	and $\rdf{w}(j) = i$.
	\begin{itemize}%[label=(4.\alph*)]
		\item If $i \ctrf{w} k$, then $j \ctrf{w} k$.
		\item If $k \ctrf{w} j$, then $k \ctrf{w} i$.
	\end{itemize}
\end{description}
\end{lemma}

\end{comment}

% \input{construction-check-order}

\input{checkorder-rf-upper-bounds}

==> checkorder-rf-upper-bounds.tex <==
%!TEX root=./main.tex

\subsection{Upper Bounds for Checking Concurrency}

In this section, we study the precise complexity of reasoning about concurrency under $\rfnovaleq$
and establish time and space upper bounds.
First, we observe that both $\checkConc{\sim}{w}{e}{f}$ and
$\checkConcSymb{\sim'}{w}{c}{d}$ can be solved using an algorithm whose
running time is a polynomial expression whose degree varies with the number of threads:


\begin{theorem}[Polynomial time algorithm]
\thmlabel{check-order-rf-time-upper-bound}
Let $w \in \alphabet$ be a run with $|w| = n$ and let 
$e, f \in \events{w}$ be two events in $w$.
The problem of determining if $\checkConc{\rfnovaleq}{w}{e}{f}$
can be solved in time $O(|\threads|\cdot n^{|\threads|+1})$.
Similarly, given $c, d \in \alphabet$, the 
problem of determining if $\checkConcSymb{\rfnovaleq}{w}{c}{d}$ can be solved in time
$O(|\threads|\cdot n^{|\threads|+2})$.
\end{theorem}

The proof of \thmref{check-order-rf-time-upper-bound} is presented
in \appref{poly-algo} and is based on constructing a 
`frontier graph'~\cite{Gibbons1994}, whose vertices represent subsets of $\events{w}$
downward closed with respect to $\po{w}$ and $\rdf{w}$,
while edges represent valid extensions obtained by single events.

We next show that the problem can also be solved using a linearly bounded Turing machine,
which also implies that
the language of runs that exhibit concurrency of two given events
is a context sensitive language.

\begin{theorem}[Linear Space Upper Bound]
\thmlabel{check-order-rf-space-upper-bound}
Let $w \in \alphabet$ be a run with $|w| = n$ and let 
$e, f \in \events{w}$ be two events in $w$.
The problem of determining if $\checkConc{\rfnovaleq}{w}{e}{f}$
can be solved in deterministic space $O(n)$.
Similarly, given $c, d \in \alphabet$, the 
problem of determining if $\checkConcSymb{\rfnovaleq}{w}{c}{d}$ 
can be solved in time deterministic space
$O(n)$.
\end{theorem}

We present the formal proof of \thmref{check-order-rf-space-upper-bound} in
 \appref{linear-space-upper-bound} and relies on successively generating permutations
 of the given run and checking if they are equivalent to the input run
 and also invert the order of the given events, all in deterministic linear space.



==> coincidence.tex <==
% !TEX root = main.tex

\section{Block Partial Order}\label{sec:bpo}
In classical trace theory, a partial order faithfully represents an equivalence class in the sense that the linearizations (aka linear extensions) of the partial order are equal to the equivalence class. As proved in \cite{bauget}, if an equivalence relation can be faithfully represented by a partial order, and if such partial orders can be appropriately concatenated, then the equivalence relations must be classic trace equivalences. This poses a serious challenge for representing a strictly weaker equivalence relation like $\beq$ by a partial order, which is the most broadly used representation of such equivalence classes in development of algorithms for verification and monitoring of concurrent programs.



%Inspired by Definition \ref{def:beq}, there is a relatively straightforward way to define a partial order that {\em corresponds} to the equivalence relation $\fbeq$. Classical trace theory associates a partial order to each equivalence class of $\meq$, where the equivalence class coincides with the set of linearizations of that partial order. Let $\hb^u$ denote the partial order that represents the equivalence class of a word $u$. 
%
%The new partial order, that represents the $\fbeq$-equivalence class of $u$, is expected to be less constrained than $\hb^u$. 
%Let $v \meq u$, and assume that a pair of blocks $B$ and $B'$ are consecutive and therefore can be swapped in $v$ to produce $v'$. This swap effectively merges the two trace equivalence classes for $v$ and $v'$.  As a result, all ordering constraints between the events of $B$ and $B'$ must be absent in our newly constructed partial order. 
%Formally, the new partial order is a subset of the intersection of $\hb^v$ and $\hb^{v'}$, which is a partial order itself. Following the same line of reasoning, the new partial order is the intersection of the partial orders obtained from all words that are reachable through valid event and block swaps outlined in Definition \ref{def:beq}. 
%
%It is however unclear how we can track all such {\em reachable} pairs of block swaps, starting from a source string $u$. Ideally, we want a partial order that can be constructed efficiently (i.e. without the need to fully or almost fully enumerate the equivalence class) from a single word $u$. 


There is a relatively straightforward way to associate a partial order to the equivalence relation $\beq$. Consider the (total) order $\hb^v$ associated to a single word $v$. The partial order associated to the equivalence class is the intersection of all the total orders associated to all words in the equivalence class. Since the intersection of any two partial orders is a partial order, this result is guaranteed to be a partial order. There are, however, two major technical obstacles for the algorithmic usage of this partial order:
\begin{enumerate}
\item This partial order does not faithfully represent the equivalence class. In fact, the set of linearizations of the order are in general is a strict superset of the equivalence class. Let 
\[v = \ev{T_1,\wt, x}\ev{T_1,\rd, x}\ev{T_2,\wt, x}\ev{T_2,\rd, x} \beq \ev{T_2,\wt, x}\ev{T_2,\rd, x}\ev{T_1,\wt, x}\ev{T_1,\rd, x}=v\]
and observe that the linearizations of the partial order associated to the equivalence class of $\{u,v\}$ includes the class and the following other four words: 
\begin{align*}
\ev{T_1,\wt, x}\ev{T_2,\wt, x}\ev{T_1,\rd, x}\ev{T_2,\rd, x}\\
\ev{T_1,\wt, x}\ev{T_2,\wt, x}\ev{T_2,\rd, x}\ev{T_1,\rd, x}\\
\ev{T_2,\wt, x}\ev{T_1,\wt, x}\ev{T_2,\rd, x}\ev{T_1,\rd, x}\\
\ev{T_2,\wt, x}\ev{T_1,\wt, x}\ev{T_1,\rd, x}\ev{T_2,\rd, x}
\end{align*}
\item It is unclear if the partial order can be computed efficiently, that is without the enumeration of the entire class. 
\end{enumerate}


In this section, we address both problems by introducing a partial order representation for $\beq$. We argue that even though the set of all linearizations of our proposed partial order may be a superset of the equivalence class (as theoretically proven to be the case in \cite{bauget}), a specific set of its linearizations, which are algorithmically easy to compute, precisely coincide with the class. Furthermore, our proposed partial order is efficiently computable. 
 
For the rest of the section, we fix a set of valid blocks $\blocks$ from which the blocks in Definition \ref{def:beq} must be chosen, and use $\fbeq$ to refer to this specialization of $\beq$ (Definition \ref{def:beq}). 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Liberal Atomicity}

A key insight of this paper is that using an appropriate notion of {\em atomicity} for the blocks paves the path to an effective definition of a partial order representation for $\fbeq$.

\begin{definition}[Liberal Atomicity]\label{def:la}
A word $v$ with a set of valid blocks $\blocks$ is called {\em liberally atomic} if there exists a word $u \fbeq v$ in which {\bf all} blocks from $\blocks$ are (contiguous) subwords of $u$. 
\end{definition}

Definition \ref{def:la} proposes a new notion of atomicity that is strictly weaker than {\em conflict-serializability} \cite{confser}. Atomicity is broadly defined as the requirement that ``there exists an {\em equivalent} run where the blocks appear serially''. Classic conflict-serializability uses $\meq$ as its underlying definition of equivalence. Liberal atomicity uses $\fbeq$ instead.  
This is the first definition of atomicity that, in terms of strictness, lies in between {\em conflict-serializability} and {\em view-serializability}, which was proven to be NP-complete to check for a single run in \cite{confser}. View-serializability uses the reads-from equivalence as its underlying notion of equivalence. Conflict-serializability, which uses trace equivalence, was then proposed as a more strict yet efficient-to-check compromise. Liberal atomicity can be viewed as being  less strict than yet equally efficient as conflict serializability. 

\begin{proposition}\label{prop:lib-atomicty}
Given a word $v$ and set of blocks $\blocks$ defined for $v$, if $v$ is conflict serializable then it is liberally atomic. The converse is not necessary true.  
\end{proposition}


The proof follows from Theorem \ref{thm:hierarchy} and Proposition \ref{prop:proper-inclusion}. Since $\fbeq$ is a superset of $\meq$, it can accordingly declare strictly more runs liberally atomic compared to conflict-serializability. The example below highlights the difference.


%\begin{example}
%  \blindtext[1]
%
%  {\makeatletter
%\let\par\@@par
%\par\parshape0
%\everypar{}\begin{wrapfigure}{r}{0.5\textwidth}
%    \framebox[0.5\textwidth]{\rule{0pt}{100pt} Figure}
%  \end{wrapfigure}
%  \blindtext[1]\par}%
%\end{example}

\parpic[r]{\includegraphics[scale=1]{figures/liberal-atomicity}}
\begin{example}\label{ex:lib-atomicity}
Let us illustrate how liberal atomicity differs from conflict-serializability. First, note that unlike most contexts in which conflict serializability is considered, our blocks need not belong to a single thread.
Consider the figure on the right. The two marked blocks on $x$ already appear serially. However, if the two operations on $z$ are also considered as a block, then the three blocks combined are not conflict-serializable.  There is a cycle in the conflict graph through the dependency edges marked with arrows. Block-equivalence, on the other hand, permits us to swap the two $x$ blocks first. Then,  $\wt(z)$ and $\rd(z)$ can be swapped against the relevant $x$ blocks to come together and appear serially. Therefore, the run with all three blocks is {\em liberally atomic}. 
\qed
\end{example}


\begin{definition}[Liberally Atomic Blocks]\label{def:wab}
A set of valid blocks $\blocks$ is called {\em liberally atomic in $v$} if every block is a distinct subsequence of $v$ and $v$ is liberally atomic if every event in $v$ that is not part of a block in $\blocks$ is treated as a singleton block.
\end{definition}



\begin{corollary}
$u \fbeq v$ implies that if a set of blocks $\blocks$ is atomic in $u$ then it is also atomic in $v$.
\end{corollary}

If a set of valid blocks $\blocks$ is liberally atomic in $v$, then any subset of it is also liberally atomic. Liberal atomicity, like conflict serializability, can be determined efficiently for a designated set of blocks $\blocks$ through a single pass over $v$. We discuss an algorithm for this in Section \ref{sec:la-alg}. Intuitively, once we limit our equivalence relation $\fbeq$ to a set of liberally atomic blocks $\blocks$, we no longer face the difficulty of figuring out which pairs of blocks from $\blocks$ can become consecutive and therefore swappable according to Definition \ref{def:beq}. Instead, liberal atomicity guarantees that any pair of blocks from $\blocks$ are swappable. This does not mean that they will necessarily be swapped. It means that if they are not otherwise ordered by more elementary constraints, i.e. the program order and read-from constraints, then it is sound to assume them swappable. 

%We define a new weaker partial order on events based the new weaker definition of atomic blocks.

\subsection{Block Happens Before}

We define a partial order on events as an analog of the classic result based on the block equivalence relation $\fbeq$. The induced partial order is always defined in the context of a specific word $w \in \Sigma_\noval^*$.

\begin{example}[A new partial order]\label{ex:bpor}
Let us outline the high level idea of this partial order before its formal exposition. Consider the concurrent program run in \figref{exbpor} with a set of marked liberally atomic blocks. Recall from Example \ref{ex:lib-atomicity} that this set of blocks is liberally atomic.
The events of thread $T_1$ that are not marked to be part of any block in the figure  have no way of being part of a valid block. The figure uses bold and thin edges. 
The union of these edges forms a minimal set of edges that capture all  constraints imposed by $\hb$ on this set of events, with the exception of the program order edges, which are assumed implicitly. There are other missing constraints, but they are implied by the transitive closure of the existing ones, for example, the conflict edge between the two $\wt(z)$ events. 

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.8]{figures/block-por}
\caption{Example \ref{ex:bpor}}\label{fig:exbpor}
\end{center}
\end{figure}


The thin edges are precisely the order constraints that our proposed {\em block happens before} relation {\em forgets}. The intuition is that the new partial order relaxes the classical ordering constraints between two blocks, because it deems them swappable. 

\parpic[r]{\includegraphics[scale=1]{figures/block-por2}}
Can this always be done soundly? No! Consider the run illustrated on the right. The set of 4 blocks is not liberally atomic (and consequently not conflict-serializable either). The pair of blocks (1) and (4) (or respectively blocks (2) and (3)) can never be in a position to be swapped. The two blocks (1) and (4) can be made serial at the same time, but then the non-serial parts of blocks (2) and (3) will be in the middle, preventing the blocks (1) and (4) to be adjacent and therefore swappable. Therefore, it is {\em unsound} to remove the conflict between the $x$ blocks (respectively the $y$ blocks). The condition of liberal atomicity for the set of blocks, rules out such unsound scenarios.  
\qed
\end{example}




% \begin{definition}[Block Happens Before $\bhb$]\label{def:bhb}
% Consider a word $w \in \Sigma_\noval^*$ and a set of liberally atomic blocks $\blocks$. Define the partial order $\bhb$ on $[0,|w|)$, parametric on $w$ and $\blocks$, as the transitive closure of the following relation ($i, j \in [0,|w|) \wedge i < j$):
% \begin{align}
% &\{ (i,j)|\ w[i] = \ev{t,o,x} \wedge w[j] = \ev{t',o',x'} \wedge \left( t = t' \vee (x = x' \wedge \wt \in \{o,o'\})\right)\}   \\ & - \{(i,j)|\ \ThreadOf{w[i]} \neq \ThreadOf{w[j]} \wedge \exists B,B' \in \blocks:\ B \neq B' \wedge w[i] \in B \wedge w[j] \in B' \}
% \end{align}
% \end{definition}
\begin{definition}[Block Happens Before $\bhb$]\label{def:bhb}
Consider a word $w \in \alphabet_\noval^*$ and a set of liberally atomic blocks $\blocks$. 
Define the partial order $\bhb$ on $\events{w}$, parametric on $w$ and $\blocks$, as the transitive closure of the following relation (event $e$ is assumed to appear before $f$ in $\tr$):
\begin{align}
&\setpred{(e,f)}{ (w[e], w[f]) \in \deprel_\noval}   \\ 
& - \setpred{(e,f)}{ \ThreadOf{e} \neq \ThreadOf{f} \wedge \exists B,B' \in \blocks:\ B \neq B' \wedge e \in B \wedge f \in B'}
\end{align}
\end{definition}



%\begin{definition}[Block Happens Before $\bhb$]\label{def:bhb}
%Consider a word $w \in \Sigma_\noval^*$ and a set of liberally atomic blocks $\blocks$. Define the partial order $\bhb$ on $[0,|w|)$, parametric on $w$ and $\blocks$, as the smallest transitive relation that satisfies the following constraints ($i, j \in [0,|w|) \wedge i < j$):
%\begin{itemize}
%\item For all $x,x' \in \vars$, $o,o' \in \set{\rd, \wt}$, $t \in \threads$: $w[i] = \ev{t,o,x} \wedge w[j] = \ev{t,o',x'}\implies i \bhb j$.
%%\item For all $x \in \vars$, $t,t' \in \threads$: $w[i] = \ev{t,\wt,x} \wedge w[j] = \ev{t',\rd,x} \wedge \rdf{w,x}(j) = i \implies i \bhb j$.
%\item For all $x \in \vars$: $\rdf{w,x}(j) = i \implies i \bhb j$.
%\item For all $x \in \vars$, $o \in \set{\rd, \wt}$, $t,t' \in \threads$: $w[i] = \ev{t,o,x} \wedge w[j] = \ev{t',\wt,x} \wedge \{i,j\} \not \subseteq \indices{w,\blocks} \implies i \bhb j$.
%\end{itemize}
%where $\indices{w,\blocks} = \{k \in [0,|w|)\ |\ \exists B \in \blocks: w[k] \in B\}$.
%\end{definition}

Note that since $\bhb$ is parametric on a word $w$ and a set of blocks $\blocks$, a verbose notation of the type $\bhbv{w}$ would best describe it. But, to keep the notation simple, we stick to $\bhb$ and note the context word $w$ whenever necessary. A transitive closure of the relation given in line (1) alone simply produces the classic trace theory partial order $\hb$. When we remove certain pairs from it through the relation given in line (2), we end up with a less constrained order relation $\bhb$. 
% Formally, the partial order is defined over the indices of the word $w$. But, with some abuse of notation, we use it between the events uniquely identified at these locations as in  $e \bhb e'$.

\begin{proposition}[Characterization of $\bhb$]\label{prop:bhb-char}
$\bhb$ is semantically sound and less constrained than $\hb$, that is: $\rdf{},\po{} \subseteq \bhb$ and $\bhb \subseteq \hb$. Furthermore, $\hb = \bhb$ if $\ \blocks = \emptyset$. 
\end{proposition}

%\begin{proposition}[Characterization of $\bhb$]\label{prop:bhb-char}
%The following four statements are true:
%\begin{itemize}
%\item $\bhb \subseteq \hb$, and if $\blocks = \emptyset$ then $\hb = \bhb$. 
%\item $RF \subseteq \bhb$.
%\item $PO \subseteq \bhb$.
%\end{itemize}
%\end{proposition}
%\azadeh{The RF/PO issue has to be settled at some point.}



\subsection{The Completeness Theorem}\label{sec:ct}

We are now ready to state the key technical result in this section, namely, that the partial order $\bhbv{w}$ precisely defines the equivalence class of $w$ up to $\fbeq$. More formally, for a fixed set of liberally atomic blocks $\blocks$, the  linearization equivalence relation $\bleq$ induced by the partial order $\bhbv{w}$ coincides with the equivalence relation $\fbeq$. Let us start by defining what equivalence classes the block partial order relation $\bhb$ defines.

\begin{definition}[Linearization Equivalence $\bleq$]\label{def:lineq}
Let $\bhb$ be defined in the context of a word $w$ and a set of blocks $\blocks$ (Definition \ref{def:bhb}). 
We say a word $u$ is a {\em proper linearization} of $\bhb$ if it is a permutation of the events from $w$ that satisfies the following two conditions:
\begin{itemize}
\item The total order of events in $u$ is consistent with the partial order $\bhb$.
\item No two blocks $B,B' \in \blocks$ where $\VariableOf{B} = \VariableOf{B'}$ overlap in $u$.
\end{itemize}
Then, $u \bleq v$ iff $u$ and $v$ are both proper linearizations of $\bhb$.
\end{definition}
By definition, $w$ itself is always a proper linearization of $\bhb$.  

\parpic[r]{\includegraphics[scale=0.9]{figures/linearization}}
\begin{example}[Proper Linearizations]\label{ex:lineq}
The partial order $\bhb$ is designed to exclude dependencies between events that {\em have the potential} to be swapped through their blocks at some point. 
The lack of a direct edge between two events, however, does not mean that they can be arbitrarily placed in a proper linearization. Consider the figure on the right. Using $\bhb$ (with $\blocks = \{1, 2, 3\}$), we take care not to directly link blocks (2) and (3). However, this does not mean that the events of these two blocks can appear in any arbitrary relative order in a proper linearization of $\bhb$. In particular, the contents of (2) and (3) cannot overlap. In any valid linearization (2) and (3) are properly ordered, but either order is acceptable.  It is fine however to arbitrarily interleave either block (2) or (3) (or both) with block (1). 
\qed
\end{example}

We now prove that the equivalence relation defined by the partial order $\bhb$, i.e. the set of its proper linearizations,  and the equivalence relation defined based on the notion of swapping of the elements from the same set of blocks $\fbeq$ coincide. First,  the easy direction:


\begin{lemma}\label{lem:lin-eq}
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$. If $u \fbeq v$ then $v$ is a proper linearization of $\bhb$, or $u \bleq v$.
\end{lemma}

It is fairly easy to reason that any single swap from Definition \ref{def:beq}, limited to the set of blocks $\blocks$, maintains the constraints of the induced partial order $\bhb$. By Definition \ref{def:bhb}, two consecutive blocks that do not share a thread cannot contain any pair of events that are related by $\bhb$. Two consecutive events that are swapped can either be operations over two different variables, or two read operations that observe the same write. Therefore, individual event swaps cannot reorder them or make two blocks accessing the same variable overlap. The proof then follows a simple inductive argument on the number of swaps. 

For the opposite direction, we need a key observation. Recall Example \ref{ex:bpor}. Consider the proper linearizations of the illustrated partial order (using bold arrows and program order constraints only). Consider the $\wt(z)$ event of $T_4$. There are no events appearing before it in the illustrated run that are causally related to it through $\bhb$. This hints at the fact that it can move backwards freely. However, it cannot move backwards to any arbitrary position. Specifically, its new position should accommodate the formation of a {\em proper} linearization. For example, it can move backward to the beginning of the run. But, it cannot move backward to be placed in the middle of the other $z$ block (with the $\wt(z)$ operation of thread $T_1$ as its head). This observation, that an unconstrained event can be swapped back in a word as long as it is guaranteed that the prefix that includes its new location can be completed to a proper linearization, is the key to proving the less trivial direction of the following theorem.


\begin{theorem}[Completeness]\label{thm:coincidence}
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$.  
We have $v \fbeq u \iff v \bleq u$. 
\end{theorem}

The completeness theorem states that the partial order $\bhb$, defined in the context of a word $u$, precisely captures the set of words that are block-equivalent to $u$ as long as the valid block swaps are limited to the set of blocks $\blocks$.

%%%%%%%%%%%%%%%%%%%%%

\subsection{Constructive Partial Order}
The definition of proper linearizations (Definition \ref{def:lineq}) and the discussion around it hints at the fact that if one is interested in a decision procedure that takes two events $e$ and $e'$ and outputs whether they can be reordered in an equivalent run, simply checking  whether $e \bhb e'$ does not provide a definitive answer. If they are ordered, then we have a negative answer. If they are not, one must yet determine if there exists a {\em proper} linearization in which they can be reordered. 

\begin{example}\label{ex:soundness}
If two events $e$ and $e'$ are not related by $\bhb$, it does not mean that they can be arbitrarily ordered. 
Consider the figure on the right. In the definition of $\bhb$, we take care not to directly link blocks (1) and (2), and similarly blocks (3) and (4). If blocks (3) and (4) disappeared, then blocks (1) and (2) could be reordered.  
\parpic[r]{\includegraphics[scale=1]{figures/soundness}}

Let us first consider the relation between blocks (3) and (4). They cannot be reordered: Since two events in blocks (3) and (4) are related through $\bhb$, the only possibility is for block (4) to appear after block (3). The reason for this is that they are blocks over the same variable, and therefore they cannot overlap. Any constraint that forces a single event of block (4) to appear after a single event of block (3), would force the entirety of block (4) to appear after the entirety of block (3). Now consider blocks (1) and (2). They can be reordered. One can break block (3), and commute block (2) (together with the $\wt(x)$ and $\rd(x)$ events of block (3) from threads $T_1$ and $T_2$) to before block (1). 

Finally, consider $\rd(z)$ of thread $T_5$ against $\wt(x)$ of thread $T_4$. They cannot be reordered, because this $\rd(z)$ is ordered before $\rd(x)$ of thread $T_4$, and reordering $\wt(x)$ of thread $T_4$ before $\rd(z)$ will amount to reordering it before $\rd(x)$ of thread $T_4$, which we have already argued is not possible.  
\qed
\end{example}


We {\em saturate} $\bhb$ with more constraints and use $\bhbs$ to represent the resulting partial order. The new partial order, which is also defined on  pairs of blocks as well as pairs of events, is the least fixed point of the following saturation rules:
\begin{align}
e \bhb e' &\longrightarrow e \bhbs e' \label{rule1}\\
\VariableOf{e} = \VariableOf{e'} \wedge e \bhbs e' &\longrightarrow B_e \bhbs B_{e'} \label{rule2} \\
B \bhbs B' &\longrightarrow \forall e \in B, \forall e' \in B':\ e \bhbs e'  \label{rule3}
\end{align}
Since $\bhb$ is a partial order, it is straightforward to conclude that so is $\bhbs$.

\begin{proposition}
$\bhbs$, as defined above, is a partial order.
\end{proposition}

Recall Example \ref{ex:soundness} and observe that $\bhbs$ relates all events of thread $T_5$ to all events of block (4), since $3 \bhbs 4$ and that makes the $\rd(x)$ of thread $T_5$ to be ordered before all events of block (4). The following lemma establishes a relation between the linearizations of $\bhb$ and $\bhbs$. 
%The proof is straightforward from the the definitions, and the observation that rules \ref{rule1,rule2,rule3} add $\bhbs$ constraints between entities that cannot be reordered.

\begin{lemma} The following are true:
\begin{enumerate}
\item Every proper linearization of $\bhb$ is a proper linearization of $\bhbs$ and vice versa.
\item If $u$ is a proper linearization of $\bhb$ (or $\bhbs$) and $v \meq u$, then $v$ is a proper linearization of $\bhbs$.
\end{enumerate}
\end{lemma}

%\azadeh{(2) will not hold for locks and must be mentioned as such}

Observe that $\bhbs$ is by definition strictly more constrained than $\bhb$, and therefore, the set of linearizations of $\bhbs$ are trivially a subset of the set of linearizations of $\bhb$. The converse is the consequence of the simple fact that every time a constraint is added to $\bhbs$ through Rules \ref{rule1},\ref{rule2}, and \ref{rule3}, no proper linearization is invalidated. The proof of the second claim is a simple consequence of the facts that $\hb \supseteq \bhbs$ and that any event swaps permitted by $\meq$ preserve the properness of a linearization.

%For the saturated partial order $\bhbs$, we can revisit the Scope Lemma, and strengthen its statement to get the following lemma.

One of the essential properties of the trace equivalence relation $\meq$ is that to determine if $vwew'$ is equivalent to  $veww'$, namely if we are asking whether $e$ can be swapped backwards against $w$, the only relevant part (the scope) is $ew$. If $ew \meq we$, then the answer is yes, and otherwise no. A complication brought about by $\rfnovaleq$ is that this nice property no longer holds. Recall the example in \figref{intro}, swapping back $\wt(x)$ would involve finding  an appropriate place for events $\wt(y)$ and $\wt(z)$ that have to move with it, and therefore would involve looking at the entirety of the illustrated run. Fortunately, we recover a version of this property for $\bhbs$, as stated by the following theorem. 

\begin{theorem}[Scope]\label{lem:sscope}
Consider a word $u$ and fix a set of liberally atomic blocks $\blocks$ for $u$ which induces the saturated partial order $\bhbs$. Let $u = v w e w'$ and assume that $v$ has the property that every block $
B \in \blocks$ is either entirely in $v$ or not at all. Moreover, assume that there is no event $f$ in $w$ such that $f \bhbs e$. Then, there exists $v'$ such that $vev'$ is a proper linearization of $\bhbs$. 
\end{theorem}

The future of $e$ has no involvement in the decision, and $v$ is only minimally involved to guarantee that $e$ is not being forced into a new position that turns the new word into something that is not a proper linearlization.

%%%




%%%%%%%%%%%%%%%%%%%%%%%%%SOUNDNESS THEOREM%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Soundness of $\bhbs$}
It remains to show that $\bhbs$ can be used in a straightforward way to decide whether two events can be reordered in an equivalent run according to $\fbeq$. First, we provide a sound algorithm to generate a proper linearization of $\bhbs$. Note that classic algorithms for {\em topological sorting} can produce linearizations of a given partial order. But, in this context, we are interested in {\em proper} linearizations, and that makes the matter slightly more complicated. 
\begin{theorem}[Proper Topological Sorting]\label{thm:tsort}
Consider a word $u$ and fix a set of liberally atomic blocks $\blocks$ for $u$ which induces the saturated partial order $\bhbs$. Let $E$ be the set of events in $u$. The following algorithm always produces a proper linearization of $E$ under $\bhbs$:
\begin{enumerate}
\item Start with $v = \epsilon$.
\item Let $e \in E$ be such that $\not \exists f \in E:\ f \bhbs e$ and that either $e$ is a read event or $\VariableOf{e}$ is not the same as the variable of any open block in $v$. 
\item Set $E = E - \{e\}$ and $v = ve$.
\item If $E \neq \emptyset$, then go to (2).
\end{enumerate}
\end{theorem}

Theorem \ref{thm:tsort} is essential for the proof of soundness, but it is also of independent interest, since it formulates under what conditions an event, whose predecessors have all been scheduled, can be soundly scheduled in a proper linearization of $\bhbs$. We provide a short proof of the Scope Theorem (Theorem \ref{lem:sscope}) using this result, and a different longer proof that does not rely on it. We are now ready to conclude with the soundness result below which states that $\bhbs$ can be used to determine if two events can be soundly reordered.

\begin{theorem}[Soundness of $\bhbs$]\label{thm:soundness}
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$, and two events $e$ and $e'$ that appear in that order in $u$. Then, $e \bhbs e'$ if and only if there does not exist a word $v \fbeq u$ in which $e'$ appears before $e$.
\end{theorem}


Let us turn our attention to the concrete problem that $\bhbs$ can solve: deciding on the status of causal concurrency of two given events $e$ and $e'$ in the context of a specific concurrent program run $u$. We can fix a set of valid liberally atomic blocks $\blocks$ in $u$ and use $\bhbs$ to decide if $e$ and $e'$ are causally ordered or concurrent wrt to $\bhbs$. However, since $\bhbs$ is parametric on $\blocks$, the answer may differ if $\blocks$ changes. Unfortunately, there exists no maximal $\blocks$ that would subsume all other choices of sets of blocks. 
\begin{wrapfigure}{r}{0.45\textwidth}
\vspace{-10pt}
\includegraphics[scale=1]{figures/block-choices}
\vspace{-10pt}
\end{wrapfigure}
Consider the concurrent program run illustrated on the right. The set of all 4 blocks marked is not liberally atomic. More specifically, any set of blocks containing the pair of blocks (1) and (2) is not liberally atomic, because only one of the two blocks can be contiguous in any equivalent run; bringing the two $x$ operations together would force the two $y$ operations apart. Blocks (1) and (3) form a liberally atomic set of blocks that consequently declare the $\wt(x)$ operation of thread $T_2$ causally concurrent to the $\wt(x)$ operation of thread $T_3$. Similarly, blocks (2) and (4) form a liberally atomic set of blocks that consequently declare the $\wt(y)$ operation of thread $T_1$ causally concurrent to the $\wt(y)$ operation of thread $T_3$. In the next section, we devise an algorithm that,  by nondeterministically choosing a set of blocks, can declare two events $e$ and $e'$ causally concurrent so long as a choice of the set of liberally atomic blocks $\blocks$ exists whose induced partial order $\bhbs$ declares them unordered. 

%
%
%So far, the notion of commutativity and the corresponding notion
%of equivalence $\fbeq$ we have been working with, is parametric
%in the choice of block $\blocks$.
%This means, for checking a property on a concurrent execution,
%one additionally needs to decide which events participate in blocks and which others do not.
%In the context of determining a property such as causal concurrency,
%a sub-optimal choice of blocks may deem two events causally ordered,
%even though a more optimal choice may deem them concurrent.
%Can we find the best choice of blocks?
%In this section, we answer this question in the positive,
%by generalizing 
%the notion of equivalence discussed so far so that it
%does retains the expressive power of block swaps, yet does not 
%rely on explicitly providing the choice of blocks.
%Our solution is to resort to \emph{all} choices of block selections.
%Towards this, we deem two executions equivalent under our new, more general, notion of equivalence,
%if they can be deemed equivalent under $\fbeq$ for any choice of $\blocks$.
%We formalize this next.


==> grain-monitor-new.tex <==
% !TEX root = main.tex
\section{Check Order Monitor}

\subsection{Sound Grain Monitor}

We assume $\alphabet_\noval$ is extended with a pair of symbols $\rhd$ and $\lhd$, 
which are used as delimiters to mark grain boundaries. 
Any letter that appears outside the range of these delimiters is treated as a standalone letter. 
For example, the word below represents 
the program run that appears in \figref{n}(a) with the marked grains:
\[
\evt{T_2}{\wt(x)} \bgn \evt{T_1}{\wt(z)} \evt{T_2}{\rd(z)} \egn \bgn \evt{T_3}{\wt(z)} \evt{T_3}{\rd(z)} \egn \evt{T_3}{\rd(x)} \bgn \evt{T_1}{\wt(x)} \evt{T_1}{\rd(x)} \egn
\]

We let the monitor check the validity of the choice of grains, 
and compute the most liberal sound commutativity relation on the fly. 
The former is a simple case of ensuring that, projected to $\bgn$ and $\egn$, 
the input string is of the form $(\bgn \egn)^*$. 
This is a regular language and can be monitored in constant space. 
Therefore, for brevity, we do not make it part of the main presentation of the monitor. 

The state of the monitor consists of the following components:
\begin{itemize}
\item $\mathit{open}$: a boolean flag that when true indicates that are in the middle of a grain.
\item $\mathit{grain}\langle V: \vars \to Bool, T: \threads \to Bool, W: \vars \to Bool, C: \vars \to Bool, F: Bool \rangle$: a tuple consisting of three maps that (respectively) remembers the set of variables accessed, the set of threads executed, and the set of variables with a write access in the grain. The last boolean value keeps track of the fact that the current grain has already been observe to be ordered wrt to a frontier node or not. 
\item $\mathit{frontier}$: a set of unique grain summaries that have been seen so far and are ordered against our source event. 
\item $NR: \vars \to Bool$: The set of variables wrt which some closed grain has nondeterministically assumed to be {\em complete}, to be checked in the future for consistency.
\end{itemize}

We define a function $\mathit{commutes}$ that takes two grains, as defined above, and returns true iff the soundly commute. 

\begin{align*}
\mathit{independent}(g_1,g_2) \iff &  g_1.T \cap g_2.T = \emptyset\ \wedge \\
                                &  g_1.V \cap g_2.V = \emptyset\ \vee \\
                                &  g_1.V \cap g_2.V \cap (g_1.W \cup g_2.W) = \emptyset\ \vee \\
                                & g_1.V \cap g_2.V \cap (g_1.W \cup g_2.W) \subseteq g_1.C \cap g_2.C 
\end{align*}

Below, we specify how the monitor updates its state, given the next input symbol. Let $g$ denote the current grain.
\begin{itemize}
\item[$\rhd$]: Set $\mathit{open}$ to true and initialize $g$ with four all false maps.
%  \begin{itemize}
%  	\item Set $\mathit{open}$ to true.
%	\item Initialize $\mathit{grain}$ with three all false maps.
%   \end{itemize}
\item[$\lhd$]: 
  \begin{itemize}
    \item If $g$ is dependent on any element of the frontier, then add $g$ to the frontier and reorganize.
    \item For every $x \in g.V$, nondeterministically set $g.C[x \mapsto \mathit{true}]$.  
    \item $NR = NR \vee g.C$ (pointwise). 
  \end{itemize}
\item[$\evt{\wt(x)}{i}$]: Set $NR[x \mapsto \mathit{false}]$. If $g.\mathit{open}$ is true then: 
  \begin{itemize}
  	\item Update $g.V[x \mapsto \mathit{true}]$ and $g.T[i \mapsto \mathit{true}]$, and $g.W[x \mapsto \mathit{true}]$. 
	\item Check if $g$ is dependent on any element of the frontier and update $g.F$ if needed.
   \end{itemize}
else: 
  \begin{itemize}
    \item Initialize $g$ with four all false maps.
  	\item Update $g.V[x \mapsto \mathit{true}]$, $g.T[i \mapsto \mathit{true}]$, and $g.W[x \mapsto \mathit{true}]$. 
	\item Nondeterministically decide to set $g.C[x \mapsto \mathit{true}]$ or skip. 
	\item Check if $g$ is dependent on any element of the frontier, add $g$ to the frontier and reorganize.
	\item $NR = NR \vee g.C$ (pointwise).
   \end{itemize}
\item[$\evt{\rd(x)}{i}$]: If $NR[x] = \mathit{true}$ then halt. 
If $\mathit{open}$ is true then: 
  \begin{itemize}
  	%\item If $g.C[x] = \mathit{true}$ and $g.W[x] = \mathit{false}$ then halt.
  	\item Update $g.V[x \mapsto \mathit{true}]$ in $g.T[i \mapsto \mathit{true}]$. 
  	\item If $g.W[x] = \mathit{false}$ then update $g.C[x \mapsto  \mathit{true}]$.
	\item Check if $g$ is dependent any element of the frontier and update $g.F$ if needed.
   \end{itemize}
else: 
  \begin{itemize}
    \item Initialize $g$ with four all false maps.
  	\item Update $g.V[x \mapsto \mathit{true}]$ and  $g.T[i \mapsto \mathit{true}]$. 
	\item Check if $g$ is dependent on any element of the frontier and update $g.F$ if needed, add $g$ to the frontier and reorganize.
   \end{itemize}
\end{itemize}


\begin{example}\label{ex:vargrains}
The run illustrated in Figure \ref{fig:n}(d) is equivalent to the one illustrated in Figure \ref{fig:n}(b), with the choice of grains as illustrated in Figure \ref{fig:n}(d); in fact, it is if we take the grains to be individual events as well. However, to argue the equivalence of the run illustrated in Figure \ref{fig:n}(d) to the one in Figure \ref{fig:n}(c), we need the $\wt(x)$ of $T_2$ to first commute as an individual event (from (d) to (b)), and then move as part of the grain that is marked in Figure \ref{fig:n}(c). Our monitor cannot keep track of these dual roles. Starting from the run illustrated in Figure \ref{fig:n}(d), it cannot see the potential of the grain including the $\wt(x)$ of $T_2$ and $\rd(x)$ of $T_3$ forming after a few sound swaps, and therefore cannot reason that $\wt(x)$ of $T_2$ can be ultimately soundly reordered against $\wt(x)$ of $T_1$. 
\end{example}

==> liberal-atomicity-algo.tex <==
%!TEX root=./main.tex

\subsection{Checking Liberal Atomicity}
\seclabel{la-alg}

We now turn our attention to the problem of checking
liberal atomicity.
Recall from \defref{la} that a word $w \in \alphabet^*$ 
is called liberally atomic with respect
to a set of blocks $\blocks$
if there is a \emph{serial} word $w'$ such that $w \fbeq w'$.

\myparagraph{Conflict Graph Characterization}{
Our first observation is that, for a given set of blocks,
one can characterize liberal atomicity in terms of acyclicity
of the graph whose nodes are blocks and edges are determined using
$\bhbs$; recall that we drop the explicit assumption of liberal atomicity on $\blocks$.
Formally, the \emph{block-graph} of $w$ and $\blocks$
is a directed graph $\graph_\blocks = (V_\blocks, E_\blocks)$
whose nodes $V_\blocks = \blocks \setpred{\set{e}}{e \in \tr, \forall B \in \blocks, e \not\in B}$
is the set of blocks and events not appearing in any block,
and whose edges are given by the order $\bhbs$ as
$E_\blocks = \setpred{(n_1, n_2)}{\exists e_1 \in n_1, e_2 \in n_2, e_1 \bhb e_2}$.
This graph precisely captures liberal atomicity:
\begin{theorem}
\thmlabel{liberal-atomicity-cycle}
Let $w \in \alphabet^*$ be a program run, $\blocks$ be a set of blocks
and let $\graph_\blocks$ be the induced block-graph.
Then, $\blocks$ is a liberally atomic set of blocks iff $\graph_\blocks$ is acyclic.
\end{theorem}
}

\myparagraph{Summarized Conflict Graph}{
While \thmref{liberal-atomicity-cycle} gives a characterization
of liberal atomicity in terms of $\bhbs$,
such a graph-based characterization is not immediately amenable to
a constant space algorithm, since linear space is required
to even construct the graph.
In order to address this concern, we consider an alternate characterization
in terms of a \emph{summarized conflict graph}~\cite{Casanova81,FM08CAV}.
% \ucomment{Define}.
Given a prefix $u$ of the run $\tr$, the summarized graph
$\sumgraph{\blocks}{u} = (V_u, E_u)$ is such that
$V_u \subseteq \blocks$ is the set of
blocks that are  \emph{active} at the end of $u$.
A block $B$ on variable $x$ is active in prefix $u$ if it is the last block
on $x$ that began in $u$.
The edges $E_u$ \emph{summarize} paths in the original conflict graph $\graph_\blocks$
\emph{through inactive transactions} --- $(B, B') \in E_u$
if there is a sequence $n_1, n_2, \ldots, n_k$ of nodes in $V_\blocks$
such that $k \geq 2$, $n_1 = B$, $n_k = B'$ $(n_i, n_{i+1}) \in E_\blocks$,
and for all $i \not\in \set{1,k}$, $n_i \not\in V_u$. 
This notion precisely captures liberal atomicity due to the following.
\begin{lemma}
\lemlabel{summarized-graph}
For a run $w \in \alphabet^*$ and blocks $\blocks$,
$\graph_\blocks$ has a cycle iff there is a prefix u of $\tr$ such that $\sumgraph{\blocks}{u}$ has a cycle.
\end{lemma}
}

\myparagraph{Finite State Automaton}{
The crucial property we exploit about the summarized 
conflict graph is that its size $|\sumgraph{\blocks}{u}|$
(for any prefix $u$) is bounded by the number 
of blocks that can be simultaneously open in any prefix 
of the string, which in turn is bounded by $|\vars|$ and thus constant.
The only missing piece is to show that
this graph can be incrementally updated.
That is, given a prefix $u$ and the next event $e$ (with $u' = ue$),
we can construct the new summary graph $\sumgraph{\blocks}{u'}$
from the summary graph $\sumgraph{\blocks}{u}$ of $u$, and some additional
constant size metadata that can guide how to updated the nodes
and edges in the graph.
Following~\cite{FM08CAV}, we design a finite state automaton:
% \[
$\autsup{\libat} = (\statessup{\libat}, \initsup{\libat}, \transsup{\libat}, \finalsup{\libat})$
% \]
}

\myparagraph{\it \underline{States of $\autsup{\libat}$}}{
There is a unique absorbing reject state $\rejsup{\libat} \in \statessup{\libat}$
for tracking if a cycle has been observed in some prefix of the run
processed by the automaton so far.
The final states are $\finalsup{\libat} = \statessup{\libat} - \set{\rejsup{\libat}}$.
A non-reject state $\ste \in \statessup{\libat} - \set{\rejsup{\libat}}$ is a tuple $q = (q_\saturated, E)$
	% \[
	% 	q = (q_\saturated, E)
	% \]
	where,
	\begin{itemize}
		\item $q_\saturated \in \statessup{\saturated}$ is a state of the saturation automaton $\autsup{\saturated}$.
		% Recall that, $q_\saturated$ in turn is a tuple
		% $q_\saturated = (\autBlks, \autRF, \autAfterSat, \autBlkAfter, \autBlkAfterOpen)$ that maintains the set of active blocks ($\autBlks$), 
		% the $\bhbs$-after set $\autAfterSat(a)$ of the latest event $e_a$
		% of each symbol $a$, 
		% and the
		% after-set $\autBlkAfter(a, t, x)$ of the first block $B$ of variable $x$ 
		% that starts in thread $t$ and is such that $e_a \bhbseq B$.
		After reading an input prefix $u$, the nodes $V_u$ of the summarized graph
		are exactly the active blocks corresponding to the domain
		of $q_\saturated.\autBlks$.
		Further, for each $x$, $q_\saturated.\autBlks(x)$ stores the contents of the active block $B_x$ on x.
		Next, for each active block $B_x$ starting at symbol $a_x$,
		the $\bhbseq$-after set of $B_x$ is precisely $q_\saturated.\autAfterSat(a_x)$.
		Finally, the maps $q_\saturated.\autBlkAfter$ together with $q_\saturated.\autBlkAfterOpen$
		can be used to infer the after sets of those nodes $n \in V_\blocks$
		such that $B_x$ to $n$ is a path in $\graph_\blocks$ and $n$ is inactive.

		\item $E \subseteq \vars \times \vars$ represents the set of edges in the summarized graph
		seen so far.
	\end{itemize}
	The initial state is $\initsup{\libat} = (\initsup{\saturated}, \emptyset)$.
}

\myparagraph{\it \underline{Transitions of $\autsup{\libat}$}}{
	Let $q = (q_\saturated, E) \in \statessup{\libat} - \rejsup{\libat}$
	and let $q' = (q'_\saturated, E') = \transsup{\libat}(q, a)$.
	First, we have $q'_\saturated = \transsup{\saturated}(q_\saturated, a)$.
	Let us see how we update the edges.
	If the incoming event $e_a$, labeled $a$, is part of an active block $B_x$ on $x$, 
	then we add the edge $(y, x)$ in one of the following cases.
	The first case is when $a \in q_\saturated.\autAfterSat(a_y)$, where $a_y$ is the unique symbol
	that starts the active block $B_y$ on $y$.
	This corresponds to the fact that there is a direct edge, between the two active blocks $B_y$ and $B_x$.
	The second case is when $a \in q_\saturated.\autBlkAfter(a_y, t, z)$
	for some $t$ and $z$.
	This corresponds to the fact that there is a summarized path from $B_y$ to $B_x$.
	If $E'$ is cyclic, then we instead set $q' = \rejsup{\libat}$.
}
The formal statement of correctness of $\autsup{\libat}$ is:
\begin{theorem}
\thmlabel{automata-la-invariant}
Let $\tr \in \alphabet^+$, $\blocks$ be a set of blocks in $\tr$
and let $\extendBlk{\tr} \in \extendBlk{\alphabet}^*$ be the corresponding annotated program run.
Let $q = \transsup{\libat}^*(\initsup{\libat}, \extendBlk{\tr})$
be the state reached by the automaton $\autsup{\libat}$ on the string $\extendBlk{\tr}$.
$q \in \finalsup{\libat}$ iff $\blocks$ are liberally atomic.
\end{theorem}

==> lower-bound-check-order.tex <==
%!TEX root = main.tex

\subsection{Lower bound for Check-Order}

We will show that there is a linear-space lower bound for Check-Order.
That is, we show that any streaming algorithm that checks for an order
between two marked events (local indices to be precise) in an input execution.


Consider the language $L_n$ for some $n$.
We describe a transducer $\Transducer_n$ such that, on input a string 
$w=a\#b$, the output $\Transducer_n(w)$ is an execution 
$\tr$ with $3$ threads $t_1$ and $t_2$, $O(n)$ events and $6$ variables such
that  $\tr$ is of the form 
\[
\tr = \pi \cdot \kappa \cdot \eta \cdot \delta
\]
The fragments $\pi$ and $\eta$ 
do not contain any access to the special variable $u$.
The fragments $\kappa$ and $\delta$ contain accesses to $u$.

Our reduction ensures the following:
\begin{enumerate}
\item If $w \in L_n$, then there are $\theta_1, \theta_2 \in \locIdxs{\tr}$ such that 
$\ThreadOf{\theta_1} = t_1, \ThreadOf{\theta_2} = t_2$, $\VariableOf{\theta_1} = \VariableOf{\theta_2} = u$ 
and $\theta_1 \ctrf{\tr} \theta_2$.
\item If $w \not\in L_n$, then there are no such $\theta_1$ and $\theta_2$.
\end{enumerate}
Moreover, $\Transducer_n$ will use $O(1)$ working space.

Let us now describe the construction of $\tr$.
At a high level, the sub-execution $\pi$ 
corresponds to the prefix $a$ of $w$ 
and the sub-execution $\eta$ corresponds to the suffix $b$ of $w$.
Both these sub-executions have $O(n)$ events.
The sub-executions $\kappa$ and $\delta$ have $O(1)$ (respectively $4$ and $1$)
events.
The sequences of events in the two sub-executions $\pi$ and $\eta$ ensure that
there is a `chain' of conditional dependencies, that
are incrementally met until the point when the two substrings $a$ and $b$ match.
If $a = b$ (i.e., full match), then the dependency chain further
ensures that there are local indices $\theta_1$ and $\theta_2$,
both in $\kappa$ (accessing the variable $u$ in threads $t_3$ and $t_2$ respectively)
such that $\theta_1 \ctrf{\tr} \theta_2$.

The execution fragment $\pi$ is of the form 
\begin{align*}
\pi = \pi_1 \cdot \pi_2 \cdots \pi_n.
\end{align*}
Here, the fragment $\pi_i$ corresponds to $a_i$ (where $a_i$ is the $i^\text{th}$ bit in $a$),
and only use the threads $t_1$.
The fragment $\eta$ is of the form
\[
\eta = \eta_1 \cdot \eta_2 \dots \eta_n \cdot \ev{t_2, \rd, u}.
\]
Here, $\eta_i$ corresponds to $b_i$ ($b_i$ is the $i^\text{th}$ bit in $b$)
and only use thread $t_2$.
The variables used in the construction are $\set{c, x_0, x_1, y_0, y_1, u}$,
where $u$ is the special variable in the definition of the problem Check-Order.
Let us now describe each of the fragments $\pi_1, \ldots, \pi_n$, $\eta_1, \ldots, \eta_n$
and the fragments $\kappa$ and $\delta$.

\myparagraph{Fragment $\pi_1$}{
	The first fragment $\pi_1$ of $\pi$ is as follows:
	\begin{align*}
	\pi_1 = \ev{t_1, \wt, x_{\neg a_1}} \cdot \ev{t_1, \wt, c} \cdot \ev{t_1, \wt, x_{a_1}}
	\end{align*}
	That is, the last (resp. first) event writes to $x_0$ (resp. $x_1$) if $a_1 = 0$, 
	otherwise it writes to the variable $x_1$ (resp. $x_0$).

	% Also observe that the read on $f$ in thread $t_3$ \emph{reads-from}\footnote{The variable $f$ will be used to enforce such \emph{reads-from} dependency n the rest of the construction too. Hence the variable name `$f$' --- reads-\underline{f}rom; we could not use `$r$' as it would be confusing, given that the symbol for a read operation is $\rd$} the write on $f$ in $t_1$.
	% That is, $\rdf{\tr}(\alpha_{\ev{t_3, \rd, f}}) = \alpha_{\ev{t_1, \wt, f}}$,
	% where $\alpha_{\ev{t_1, \rd, f}}$ is the local index of the unique symbol $\ev{t_3, \rd, f}$ in $\pi_1$,
	% and $\alpha_{\ev{t_1, \wt, f}}$ is defined in a similar fashion.
	% We will use the following shorthand notation to denote this :
	% \begin{align*}
	% \rdf{\tr}(\ev{t_3, \rd, f, \pi_1}) = \ev{t_1, \wt, f, \pi_1}
	% \end{align*}
	% In the above, the last argument $\pi_1$ disambiguates the local indices, 
	% as there will be other reads and writes on $f$ in later fragments.
	% Observe that due to this, $\alpha_{\ev{t_1, \wt, f}} \trf{\tr} \alpha_{\ev{t_3, \rd, f}}$.
	% We denote by the shorthand $\ev{t_1, \wt, f, \pi_1} \trf{\tr} \ev{t_3, \rd, f, \pi_1}$,
	% Also observe that
	% $\rdf{\tr}(\ev{t_1, \rd, f, \pi_1}) = \ev{t_3, \wt, f, \pi_1}$
	% and thus $\ev{t_3, \wt, f, \pi_1} \trf{\tr} \ev{t_1, \rd, f, \pi_1}$.
	% This reads-from dependency, in turn ensures that
	% $\ev{t_3, \wt, c, \pi_1} \trf{\tr} \ev{t_1, \wt, x_{a_1}, \pi_1}$.
}

\myparagraph{Fragment $\eta_1$}{
	The first fragment $\eta_1$ of $\eta$ is as follows:
	\begin{align*}
	\eta_1 = \ev{t_2, \rd, x_{b_1}} \cdot \ev{t_2, \wt, c}
	\end{align*}

	In the entire construction, the variables $x_0$ and $x_1$ are being written-to only
	in fragment $\pi_1$, and (potentially) read only in $\eta_1$.
	This means that, either $\rdf{\tr}(\ev{t_2, \rd, x_{b_1}, \eta_1}) = \ev{t_1, \rd, x_{a_1}, \pi_1}$
	(if $a_1 = b_1$)
	or $\rdf{\tr}(\ev{t_2, \rd, x_{b_1}, \eta_1}) = \ev{t_1, \rd, x_{\neg a_1}, \pi_1}$
	(if $a_1 \neq b_1$)\footnote{Here, we use the notation $\ev{t, o, v, \gamma}$ 
	to denote the unique local index $\alpha$ in the fragment $\gamma$ for which $\tr[\alpha] = \ev{t, o, v}$.}.
	If $a_1 = b_1$, then we further have
	$\ev{t_1, \wt, c, \pi_1} \trf{\tr} \ev{t_2, \wt, c, \eta_1}$.
	That is,
	\begin{align}
	\equlabel{pi1_c_to_eta1_c}
	a_1 = b_1 \implies \ev{t_1, \wt, c, \pi_1} \trf{\tr} \ev{t_2, \wt, c, \eta_1}
	\end{align}
}

\myparagraph{Fragment $\pi_i$ ($i \geq 2$)}{
For each $i\geq 2$, the fragment $\pi_i$ is the following
\begin{align*}
	\pi_i = \ev{t_1, \wt, y_{a_i}}  \cdot \ev{t_1, \rd, c} \cdot \ev{t_1, \wt, c} \cdot \ev{t_1, \wt, r_{a_i}}.
\end{align*}	
Let us list some reads-from dependencies introduced due to $\pi_i$ ($i \geq 2$):
\begin{align*}
	\begin{array}{lcr}
		\rdf{\tr}(\ev{t_1, \rd, y_{a_2}, \pi_i}) &=& \ev{t_1, \wt, y_{a_2}, \pi_i} \\
		\rdf{\tr}(\ev{t_3, \rd, c, \pi_i}) &=& \ev{t_3, \wt, c, \pi_{i-1}} \\
	\end{array}
\end{align*}
Recall from \equref{pi1_c_to_eta1_c} that, if $(a_1 = b_1)$, then $\ev{t_1, \wt, c, \pi_1} \trf{\tr} \ev{t_2, \wt, c, \eta_1}$.
Also because $\rdf{\tr}(\ev{t_1, \rd, c, \pi_2}) = \ev{t_1, \wt, c, \pi_1}$, 
by the definition of closure (\defref{conflicting-closure}), we further have
$\ev{t_1, \rd, c, \pi_2} \ctrf{\tr} \ev{t_2, \wt, c, \eta_1}$ 
dependency\footnote{The variable $c$ is thus used to enforce dependencies due to `conflicting-\underline{c}losure'; hence the name `c'.}.
Finally, the read-from dependency from $t_1$ to $t_3$ due to $f$ gives us:
\begin{align}
\equlabel{pi2_a2_to_eta1_c}
a_1 = b_1 \implies \ev{t_1, \wt, y_{a_2}, \pi_2} \ctrf{\tr} \ev{t_2, \wt, c, \eta_1}
\end{align}
}



\myparagraph{Fragment $\eta_i$ ($i \geq 2$)}{
For each $i\geq 2$, the fragment $\eta_i$ is the following
\begin{align*}
	\eta_i = \ev{t_2, \wt, y_{b_i}} \cdot \ev{t_2, \wt, c}.
\end{align*}
It is easy to see from \equref{pi2_a2_to_eta1_c} that if $a_1 = b_1$
then the thread-order dependency between $\eta_1$ and $\eta_2$
further gives us
$\ev{t_1, \wt, y_{a_2}, \pi_2} \ctrf{\tr} \ev{t_2, \wt, y_{b_2}, \eta_2}$.
Now, if additionally $a_2 = b_2$, we can again invoke \defref{conflicting-closure}
and get:
\begin{align}
\equlabel{pi2_a2_to_eta2_b2}
(\forall i \leq 2, a_i = b_i) \implies \ev{t_1, \rd, y_{a_2}, \pi_2} \ctrf{\tr} \ev{t_2, \wt, y_{b_2}, \eta_2}
\end{align}.

In fact, the same reasoning can be inductively extended for any $2 \leq k \leq n$:
\begin{align}
\equlabel{pii_ai_to_etai_bi}
(\forall i \leq k, a_i = b_i) \implies \ev{t_1, \rd, y_{a_k}, \pi_k} \ctrf{\tr}  \ev{t_2, \wt, y_{b_k}, \eta_k}.
\end{align}
The base case of $k=2$ follows from \equref{pi2_a2_to_eta2_b2}.
For the inductive case, assume that the statement holds for some $k < n$.
Also assume the antecedent is true, i,e., $(\forall 2 \leq i \leq k, a_i = b_i)$.
This means that $\ev{t_1, \rd, y_{a_k}, \pi_k} \ctrf{\tr} \ev{t_2, \wt, y_{b_k}, \eta_k}$.
This further means that $\ev{t_1, \wt, c, \pi_k} \ctrf{\tr} \ev{t_2, \wt, c, \eta_k}$
by composition with thread order.
Then, by \defref{conflicting-closure}, we get
$\ev{t_1, \wt, c, \pi_{k+1}} \ctrf{\tr} \ev{t_2, \wt, c, \eta_k}$.
This, in turn implies that $\ev{t_1, \wt, y_{a_{k+1}}, \pi_{k+1}} \ctrf{\tr} \ev{t_2, \wt, y_{b_{k+1}}, \eta_{k+1}}$.
Now, assume that $a_{k+1} = b_{k+1}$.
Then, by  \defref{conflicting-closure}, we get 
$\ev{t_1, \rd, y_{a_{k+1}}, \pi_{k+1}} \ctrf{\tr} \ev{t_2, \wt, y_{b_{k+1}}, \eta_{k+1}}$,
as desired.
}

\myparagraph{Fragments $\kappa$ and $\delta$}{
	The sequence $\kappa$ is:
	\begin{align*}
		\kappa = \ev{t_1, \wt, u} \cdot \ev{t_1, \rd, c} \cdot \ev{t_1, \rd, u} \cdot \ev{t_2, \wt, u}.
	\end{align*}
	The fragment $\delta$ is the singleton sequence:
	\begin{align*}
		\delta = \ev{t_2, \rd, u}
	\end{align*}

	The reads-from dependencies induces due to $\kappa$ and $\delta$ are:
	\begin{align*}
	\begin{array}{lcr}
		\rdf{\tr}(\ev{t_1, \rd, c, \kappa}) &=& \ev{t_1, \wt, c, \pi_n} \\
		\rdf{\tr}(\ev{t_1, \rd, u, \kappa}) &=& \ev{t_1, \wt, u, \kappa} \\
		\rdf{\tr}(\ev{t_2, \rd, u, \delta}) &=& \ev{t_2, \wt, u, \kappa} \\
	\end{array}
	\end{align*}
}

\figref{check-order-lb-trace} describes our construction for $n=4$.

\input{figures/lowerbound-check-order}

\myparagraph{Correctness}{
	Let us make some simple observations.
	First, every read event has a write event on the same variable prior to it; hence
	$\tr$ is a consistent execution.
	Second, it is easy to see that the construction can be performed by a transducer
	$\Transducer_n$ in $O(1)$ space.

	($\Rightarrow$)
	Let us first prove that if $\forall i \in [n], a_i = b_i$, then $\theta_1 \ctrf{\tr} \theta_2$,
	where $\theta_1$ is the local index of the $\ev{t_1, \rd, u}$ event in $\kappa$
	and $\theta_2$ is the local index of the $\ev{t_2, \wt, u}$ event in $\kappa$.
	% Assume $\forall i \in [n], a_i = b_i$.
	% From \equref{pii_ai_to_etai_bi}, we have $\ev{t_1, \rd, y_{a_n}, \pi_n} \ctrf{\tr} \ev{t_2, \wt, y_{b_n}, \eta_n}$.
	% Then, by transitivity of $\ctrf{\tr}$, we get
	% $\ev{t_3, \wt, c, \pi_n} \ctrf{\tr} \ev{t_2, \wt, c, \eta_n}$
	% and finally  $\theta_1 \ctrf{\tr} \ev{t_2, \rd, u, \tr_3}$
	% Then by \defref{conflicting-closure}, we get
	% $\theta_1 \ctrf{\tr} \theta_2$.
	Recall that if $a_i = b_i$ for every $i\leq n$, then 
	$\ev{t_3, \rd, y_{a_n}, \pi_n} \ctrf{\tr}  \ev{t_2, \wt, y_{b_n}, \eta_n}$
	(see \equref{pii_ai_to_etai_bi}).
	As a result, $\ev{t_1, \wt, c, \pi_n} \ctrf{\tr}  \ev{t_2, \wt, c, \eta_n}$.
	Next, due to \defref{conflicting-closure}, we get
	$\ev{t_1, \rd, c, \kappa} \ctrf{\tr}  \ev{t_2, \wt, c, \eta_n}$.
	This, together with thread-order further gives
	$\ev{t_1, \wt, u, \kappa} \ctrf{\tr}  \ev{t_2, \rd, u, \delta}$.
	If we next apply \defref{conflicting-closure}, we get
	$\ev{t_1, \wt, u, \kappa} \ctrf{\tr}  \ev{t_2, \wt, u, \kappa}$.
	Applying \defref{conflicting-closure} once again, we get
	$\theta_1 = \ev{t_1, \rd, u, \kappa} \ctrf{\tr}  \ev{t_2, \wt, u, \kappa} = \theta_2$.
	% In summary, 
	% \begin{align}
	% \equlabel{r_u_kappa_to_w_u_kappa}
	% (\forall i \leq n, a_i = b_i) \implies \ev{t_3, \rd, u, \kappa} \ctrf{\tr}  \ev{t_2, \wt, u, \kappa}.
	% \end{align}

	($\Leftarrow$)
	Let us now prove that if there is an index $i$ for which $a_i \neq b_i$, 
	then for the local indices $\theta_1$ and $\theta_2$
	corresponding to $\tr[\theta_1] = \ev{t_1, \rd, u}$
	and $\tr[\theta_2] = \ev{t_2, \wt, u}$, we have
	$\theta_1 \notctrf{\tr} \theta_2$ and $\theta_2 \notctrf{\tr} \theta_1$.
	To show this, we will construct an execution $\tr'$ such that
	$\tr' \sim \tr$ and $\theta_2 \trord{\tr'} \theta_1$,
	and then by \propref{equivalence-preserves-ctrf}, we will have
	$\theta_1 \notctrf{\tr} \theta_2$ and $\theta_2 \notctrf{\tr} \theta_1$.
	In the rest, we assume $i$ is the least such index.


	First, consider the case when $i = 1$. 
	In this case, $\neg a_1 = b_1$.
	Then, $\tr'$ is the following concatenated sequence ($\kappa'$ is the second largest prefix of $\kappa$):
	\[
		\tr' = \ev{t_2, \wt, u} \cdot \ev{t_1, \wt, x_{\neg a_1}} \cdot \eta \cdot \delta \cdot \ev{t_1, \wt, x} \cdot \ev{t_1, \wt, x_{a_1}}\cdot \pi_2 \cdots \pi_n \cdot \kappa'
	\]
	First, observe that, the thread-wise projections of $\tr$ and $\tr'$ are the same
	and thus $\tho{\tr} = \tho{\tr'}$.
	Next, we note thar the reads-from dependencies of each read access to either $y_0, y_1, c$ or $u$
	are the same in both $\tr$ and $\tr'$:
	\begin{itemize}
		\item The only read accesses to $y_0$ or $y_1$ are in thread $t_1$, and so are their corresponding write events (as per $\tr$). In the new sequence $\tr'$, we ensure that
		all write access to $y_0$ or $y_1$ in $t_2$ occur before any access to $y_0$ or $y_1$
		in thread $t_1$.
		\item The same reasoning as above applies to the accesses to $c$.
		\item The read access to $u$ in $t_2$ appears before the write access to $u$ in $t_1$ in the new sequencd $\tr'$.
	\end{itemize}
	Finally, the reads-from dependency of $\ev{t_2, \rd, x_{b_1}}$ is also preserved. 
	Hence, $\tr'\sim\tr$.
	Finally, observe that the local indices $\theta_2 = \ev{t_2, \rd, u, \kappa}$
	and $\theta_1 = \ev{t_1, \wt, u, \kappa}$ are such that $\theta_2 \trord{\tr'} \theta_1$.

	Next, consider the case of $i > 1$.
	Then, we construct $\tr'$ as the following interleaved sequence:

	\[
		\gamma_1 \cdot \gamma_2 \cdots \gamma_n \cdot \kappa'
	\]
	where:
	\begin{align*}
	\begin{array}{rclr}
	\gamma_1 &=& \ev{t_2, \wt, u} \cdot \ev{t_1, \wt, x_{\neg a_1}} \cdot \ev{t_1, \wt, c} \cdot \ev{t_1, \wt, x_{a_1}} \cdot \ev{t_2, \rd, x_{b_1}} & \\
	\gamma_j &=& \ev{t_1, \wt, y_{a_j}} \cdot \ev{t_1, \rd, c} \cdot \ev{t_2, \wt, c} \cdot \ev{t_1, \wt, c} \cdot \ev{t_1, \rd, y_{a_j}} \cdot \ev{t_2, \wt, y_{b_j}} & 2 \leq j < i \\
	\gamma_i &=& \ev{t_1, \wt, y_{a_i}} \cdot \ev{t_1, \rd, c} \cdot \ev{t_2, \wt, c} \cdot \ev{t_2, \wt, y_{b_i}} \cdot \ev{t_2, \wt, c} \cdot \ev{t_1, \wt, c} \cdot \ev{t_1, \rd, y_{a_i}}  & \\
	\gamma_j &=& \ev{t_2, \wt, y_{b_j}} \cdot \ev{t_1, \wt, y_{a_j}} \cdot \ev{t_1, \rd, c} \cdot \ev{t_2, \wt, c} \cdot \ev{t_1, \wt, c} \cdot \ev{t_1, \rd, y_{a_j}} & j > i \\
	\kappa' &=& \ev{t_2, \rd, u} \cdot \ev{t_1, \wt, u} \cdot \ev{t_1, \rd, c} \cdot \ev{t_1, \rd, u} & \\
	\end{array}
	\end{align*}


	Here again, we observe that the new trace $\tr'$ is such that $\tho{\tr} = \tho{\tr'}$,
	and further, for every read access, the write accesses are the same local indices in both $\tr$ and $\tr'$.
	That is, $\tr \sim \tr'$.
	Further, observe that the positions of $\theta_1$ and $\theta_2$ have been inverted.
	This trace $\tr'$ for a special case is shown in \figref{check-order-lb-reordering}.

	This finishes our proof.
}

\begin{remark}
The above proof also shows that there is a linear space lower bound for streaming algorithms of the following problem:
\begin{problem}[Check-Singleton]
Given a consistent execution $\tr \in \Sigma^+$, 
check if there is no other consistent execution $\tr' \neq \tr$
such that $\tr \sim \tr'$.
That is, the problem asks to check if the equivalence class of $\tr$ is singleton.
\end{problem}
The hardness follows from the observation that the $\ctrf{\tr}$
order of the constructed execution is a total order iff the
the $a = b$ in the input instance for the language $L_n$.
\end{remark}

\subsection{Linear space lower bound for checking normal forms}

The construction for the space lower bound for Check-Order can
be directly lifted for showing the lower bound for Check-FNF and Check-LexNF.
As before, the reduction is from $L_n$
and the execution we construct is the same execution $\tr$ as before.
We fix the order $<_{\threads}$ as $t_2 <_\threads t_1$.

If $a = b$, then $\theta_1 \ctrf{\tr'} \theta_2$
for every $\tr' \sim \tr$.
In this case, $\tr$ is both the Lexicographic and Foata Normal Form.

Otherwise, the execution $\tr'$ that we construct to show $\theta_1 \notctrf{\tr} \theta_2$
witnesses that $\tr$ is neither the Lexicographic normal form,
nor the Foata normal form.

\begin{theorem}
Both $L_{\foatanf}$ and $L_{\lexnf}$ are non-regular languages.
\end{theorem}

==> maz-block-combo.tex <==
% !TEX root = main.tex

\section{Block Partial Order}\label{sec:bpo}

There are at least 3 different canonical forms of representing the well-studied Mazurkiewicz trace equivalence classes in the literature: lexicographical normal forms \cite{..}, Foata normal forms, and Hasse Diagrams \cite{...}. The latter is the most broadly known representation for these equivalences in which a {\em partial order} represents an equivalence class, and each member of the class is in turn a {\em linearization} of this partial order. There is work in the literature \cite{...} on how such a representation can be a useful algorithmic tool for problems like race detection \cite{...}. In this section, we introduce an analogous partial order representation for $\beq$. 

\begin{definition}[Atomic Blocks]
A subsequence of a word $v$ is called an {\em atomic block} in $v$ if there exists a word $u$ such that $u \meq v$ and the subsequence is a subword of $u$. A set of blocks $\blocks$ is called {\em atomic in $v$} if every block is a distinct subsequence of $v$ and there exists a word $u \meq v$ in which {\bf all} blocks from $\blocks$ are subwords of $u$.
\end{definition}

This definition coincides with the classic definition of {\em conflict-serializability} \cite{cf}. In other words, we call a set of blocks atomic iff they are conflict serializable. 

\begin{corollary}
Consider the set of blocks $\blocks$ as transactions, and the remaining events in $w$ that do not belong to any block as singleton transactions. $\blocks$ is atomic iff $w$ is conflict serializable with the corresponding choice of transactions.
\end{corollary}


\begin{proposition}\label{prop:maz-blocks}
$u \meq v$ implies that if a set of blocks $\blocks$ is atomic in $u$ then it is also atomic in $v$.
\end{proposition}

\begin{proposition}\label{prop:noreturn}
$u \beq v$ {\bf does not} imply that a set of blocks $\blocks$ that is atomic in $u$ is also atomic in $v$.
\end{proposition}
\begin{proof}
\begin{center}
\includegraphics[scale=0.13]{figures/ce1}
\end{center}
\end{proof}


We define a partial order on events as an analog of the classic result based on the block equivalence relation $\beq$. The induced partial order is always defined in the context of a word $w \in \Sigma_\noval^*$. We fix a set of valid blocks $\blocks$ from which the blocks from Definition \ref{def:beq} must be chosen. We use the alternate symbol $\fbeq$ to indicate the variation of Definition \ref{def:beq} that is parametric on $\blocks$. 

\begin{definition}[Block Happens Before $\bhb$]\label{def:bhb}
Consider a word $w \in \Sigma_\noval^*$ and a set of atomic blocks $\blocks$. Define the partial order $\bhb$ on $[0,|w|)$, parametric on $w$ and $\blocks$, as the smallest transitive relation that satisfies the following constraints ($i, j \in [0,|w|) \wedge i < j$):
\begin{itemize}
\item For all $x,x' \in \vars$, $o,o' \in \set{\rd, \wt}$, $t \in \threads$: $w[i] = \ev{t,o,x} \wedge w[j] = \ev{t,o',x'}\implies i \bhb j$.
%\item For all $x \in \vars$, $t,t' \in \threads$: $w[i] = \ev{t,\wt,x} \wedge w[j] = \ev{t',\rd,x} \wedge \rdf{w,x}(j) = i \implies i \bhb j$.
\item For all $x \in \vars$: $\rdf{w,x}(j) = i \implies i \bhb j$.
\item For all $x \in \vars$, $o \in \set{\rd, \wt}$, $t,t' \in \threads$: $w[i] = \ev{t,o,x} \wedge w[j] = \ev{t',\wt,x} \wedge \{i,j\} \not \subseteq \indices{w,\blocks} \implies i \bhb j$.
\end{itemize}
where $\indices{w,\blocks} = \{k \in [0,|w|)\ |\ \exists B \in B: w[k] \in B\}$.
\end{definition}
Note that since $\bhb$ is parametric on $w$ and $\blocks$, a verbose notation of the type $\bhb_{w,\blocks}$ would best describe it. But, to keep the notation simple, we stick to $\bhb$ and note the parameters whenever necessary. 

\begin{proposition}[Characterization of $\bhb$]\label{prop:bhb-char}
The following three statements are true:
\begin{itemize}
\item $\bhb \subseteq \hb$, and if $\blocks = \emptyset$ then $\hb = \bhb$. 
\item $RF \subseteq \bhb$.
\item $PO \subseteq \bhb$.
\end{itemize}
\end{proposition}


\begin{definition}[Linearization Equivalence $\bleq$]
Let $\bhb$ be defined in the context of a word $w$ and a set of blocks $\blocks$ (Definition \ref{def:bhb}). 
We say a word $u$ is a {\em proper linearization} of $\bhb$ if it is a linear sequence of the events from $w$ that satisfies the following two conditions:
\begin{itemize}
\item The total order of events in $u$ is consistent with the partial order $\bhb$.
\item No two blocks $B,B' \in \blocks$ where $\VariableOf{B} = \VariableOf{B'}$ overlap in $u$.
\end{itemize}
$u \bleq v$ iff $u$ and $v$ are both proper linearizations of $\bhb$.
\end{definition}
By definition, $w$ itself is always a proper linearization of $\bhb$. 

\subsection{The Representation Theorem}\label{sec:ct}

\begin{lemma}\label{lem:maz-lin}
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$. If $u \meq v$ then $v$ is a proper linearization of $\bhb$.
\end{lemma}
The proof is a direct consequence of Lemma \ref{prop:maz-blocks}, which states that the blocks $\blocks$ remain atomic in $v$ and the definition of atomicity of $\blocks$ which implies that $\meq$ preserves their atomicity.  


\begin{remark}\label{rem:lin-ce}
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$. If $u \beq v$ then $\blocks$ do not necessarily remain atomic in $v$ and therefore, the order $\bhb$ may be ill-defined in $v$.
\end{remark}

This is a direct consequence of Proposition \ref{prop:noreturn}. 

\begin{lemma}[Scope]\label{lem:scope}
Consider a word $u$ and fix a set of atomic blocks $\blocks$ for $u$ which induces the partial order $\bhb$. Let $u = v w e w'$ and assume that $w$ contains no event $f$ where $f \bhb e$ and $v$ does not end in the middle of a block $B \in \blocks$ where $\VariableOf{B} = \VariableOf{e}$ unless $e \in B$. Then, there exists a word $v'$ such that  $u \fbeq vev'$. 
%and $u \bleq vev'$
%if no two blocks over the same variable overlap in $vev'$.
\end{lemma}
%%%
\begin{proof}
We show that $e$ can be swapped backwards in $w$ until it reaches the beginning of $w$ as follows. In each case, we also argue that, after each step, the resulting word $u'$ satisfies $u \fbeq u'$.
\begin{itemize}
\item[(i)] If $w$ only contains events that access a variable other than $\VariableOf{e}$, and considering that by definition of $\bhb$ we know that no event in $w$ shares a thread with $e$, we can conclude that  $e$ does commute against every event in $w$. Therefore, $v w e w' \meq v e w w'$. By Theorem \ref{thm:hierarchy}, we can conclude that $vwew' \fbeq veww'$.
%Besides, all the single event swaps, by Lemma \ref{lem:maz-lin}, preserve $\bleq$.

\item[(ii)] If $w$ contains events $f$ such that $\VariableOf{f} = \VariableOf{e}$, then by the definition of $\bhb$,  $e$ and all such $f$'s must be part of a block in $\blocks$. First, we consider the location of $e$ in its block $B_e$. It can be the first event of $B_e$.  If not, then $e'$ is the first event of $B_e$ and we have $e' \bhb e$. Therefore, $e'$ cannot be in $w$. But, it must have appeared before $e$ in $u$, and therefore it must be in $v$. But then, by definition, all events accessing $\VariableOf{e}$ in $w$ must belong to $B_e$ as well. Since these are all $\rd$ events and none of them can share a thread with $e$, this case defaults back to case (i) where $e$ can be swapped back over all such events, and $v e w w'\meq v w e w'$. Therefore, we proceed assuming that $e$ is the first event of $B_e$. We argue using the following steps:
\begin{itemize} 
    \item Since in $vwew'$ no two blocks over he same variable overlap, we can conclude that all events $f$ over the $\VariableOf{e}$ in $w$ are part of blocks that begin and end in $w$. If not, one such block would begin in $v$ and end in $w$, which is a contradiction.
	\item By the definition of atomic blocks, we know there exists a word $\sigma \meq wew'$ such that the block of $e$ and all events $f$ in $w$ that access $\VariableOf{v}$ appear serially in $\sigma$. By Theorem \ref{thm:hierarchy}, $v\sigma \fbeq u$.
	\item In $v \sigma$, we can swap back $B_e$ to the beginning of $\sigma$, since everything on its way either is an independent event accessing another variable or a block accessing $\VariableOf{v}$. The resulting word $v B_e \sigma'$ clearly satisfies $v B_e \sigma' \fbeq v\sigma$.  
	%\item All the single event swaps, by Lemma \ref{lem:maz-lin}, preserve $\bleq$. It remains to argue that the swaps of block $B_e$ also preserve $\bleq$, because generally the swap of any pair of blocks does not (Remark \ref{rem:lin-ce}).  The reason is that once $B_e$ sits at the beginning of $\sigma$, any (new) conflict edges that it incurs cannot participate in the formation of any cycle. Therefore, blocks that are conflict serializable before, remain conflict serializable after.

 
\end{itemize}
\end{itemize}

\end{proof}



\begin{theorem}[Representation]
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$. If $v \fbeq u$ then $v \fbeq u$. 
\end{theorem}

\begin{proof}
We prove that we can {\em bubble sort} $u$ to get $v$, using the two types of swaps that are outlined in Definition \ref{def:beq}. Starting from the index $0$, we identify the location of the next $v[i]$ in $u$ and swap it backwards to position $i$. Formally, we prove by induction that for all index $i$, $v[i]$ can be successfully placed after $v[0] \dots v[i-1]$ have been placed, to produce an intermediate string $v'$ where $v' \fbeq u$ and $v' \bleq u$.

Base Case: Let $i = 0$. Let $v[0] = e$ and $u = s e t$. By definition of $\bhb$ and the fact that $v \bleq u$, we know there exists no event $f$ in $u$ or $v$ (specifically in $s$) such that $f \bhb e$. Using Lemma \ref{lem:scope}, we argue that $e$ can be swapped back to the beginning of the word. Lemma \ref{lem:scope} suggests a word $u' \fbeq u$ where $e$ appears at the beginning of $u'$. 

We additionally need to argue that $u' \bleq u$. All the single event swaps, by Lemma \ref{lem:maz-lin}, preserve $\bleq$. It remains to argue that the swaps of block $B_e$, in the proof of Lemma \ref{lem:scope} also preserve $\bleq$, because generally the swap of any pair of blocks does not (Remark \ref{rem:lin-ce}).  The reason is that once $B_e$ sits at the beginning of $u'$, any (new) conflict edges that it incurs cannot participate in the formation of any cycle. Therefore, blocks that are conflict serializable before, remain conflict serializable after.


%We swap $e$ backwards in $u$ until it reaches the beginning of the word as follows. In each case, we also argue that for the resulting word $w$, we have $w \bleq u$.
%\begin{itemize}
%\item[(i)] If $s$ only contains events that access a variable other than $\VariableOf{e}$, then by definition of $\bhb$ we know that no event in $s$ shares a thread with $e$ either. Therefore, $e$ does commute against every event in $s$. By construction, $e s t \meq s e t$. By Theorem \ref{thm:hierarchy}, we can conclude that $s e t \fbeq e s t$.
%\item[(ii)] If $s$ contains events $f$ such that $\VariableOf{f} = \VariableOf{e}$, then by the definition of $\bhb$,  $e$ and all such $f$'s must be part of a block in $\blocks$.
%\begin{itemize}
%	\item By the definition of atomic blocks, we know there exists a word $w \meq u$ such that the block of $e$ and all such $f$'s appear serially in $w$. By Lemma \ref{lem:maz-lin}, $w \bleq u$. By Theorem \ref{thm:hierarchy}, $w \fbeq u$.
%	\item We start with $w = s B_e t$, where $B_e$ is the block from $\blocks$ that contains $e$. We swap $B_e$ back to the beginning. Note that by definition of $e$, there cannot exist an event $f$ in $s$ such that $f \bhb e$, and $e$ is the first event of $B_e$. Like the previous case, $B_e$ commutes against everything in $s$ and can be swapped to the beginning, placing $e$ at the right location. Note that to form the serial blocks, all the swaps are for a pair of events over two different variables. Therefore, $s$ will contain serial blocks over $\VariableOf{e}$ and otherwise events over other variables. $B_e$ commutes against all other serial blocks over $\VariableOf{e}$, because otherwise, it must share a thread with them and that violates the existence of a string $v \bleq u$ with $e$ as its first event. Blocks over the same variable never overlap, which means in $v$ the block of $e$ has to appear before this other block which has an event in it that is ordered before an event of $B_e$ through $\bhb$. 
%	\item It remains to argue that $B_e s t \bleq u$. All the single event swaps, by Lemma \ref{lem:maz-lin}, preserve the equivalence. But, not all block swaps do. But, the swap of $B_e$ does. The reason is that once $B_e$ sits at the beginning, any (new) conflict edges that it incurs cannot participate in the formation of any cycle. Therefore, blocks that are conflict serializable before, remain conflict serializable after.
%\end{itemize}
%\end{itemize}



The Induction Hypothesis: Let us assume we can place the first $n - 1$ symbols of $v$ through swaps. Let $\alpha$ be the prefix of $v$ of length $n - 1$. Let $w = \alpha s e t$. We know that  $w \fbeq u$, $\blocks$ are valid atomic blocks of $w$  and $w$ is a proper linearization of $\bhb$.

The goal is to show that we can swap $e = v[n]$ into place and satisfy the induction hypothesis. As before, we know that no event $f$ in $s$ satisfies $f \bhb e$. Using Lemma \ref{lem:scope}, we can argue why $e$ or its block can be commuted back and placed right after $\alpha$ resulting a new word $u'$. 

We additionally need to argue that $u' \bleq u$. All the single event swaps, by Lemma \ref{lem:maz-lin}, preserve $\bleq$. It remains to argue that the swaps of block $B_e$, in the proof of Lemma \ref{lem:scope} also preserve $\bleq$.  The reason is that once $B_e$ sits right after $\alpha$, any (new) conflict edges that it incurs cannot participate in the formation of any cycle for blocks that appear after it in $u'$. Therefore, blocks that will participate in the continuation of this inductive argument will remain conflict serializable as before.


% 
%\begin{itemize}
%\item If $s$ only contains events that access a variable other than $\VariableOf{e}$, then the argument is identical to that of the case (i) of the base case.
%\item If $s$ contains accesses to $\VariableOf{e}$, then the argument is similar to case (ii) of the base case. In particular:
%\begin{itemize}
%	\item One can argue that $e$ must be the first event of its corresponding block $B_e$.  
%	\item All other blocks $B$ over $\VariableOf{e}$ are entirely included in $s$. This is because blocks over the same variable are never nested in a proper linearization by definition, and therefore, parts of these blocks cannot be in $t$. They cannot be in $\alpha$ because then the placement of $e$ at the end of $\alpha$ would land it in the middle of one such block and therefore violate the condition that $v$ is a proper linearization.
%	\item $t$ can only contain the remainder of the block of $e$. 
%	\item We start with serializing all blocks in $s$ over $\VariableOf{e}$ and the block of $e$ as well. The argument why $B_e$ can then commute to the beginning of $s$ is identical to case (ii) of the base case. 
%\end{itemize}	
%\end{itemize}	
\end{proof}

\begin{theorem}[Soundness of $\bhb$]
Consider a word $u$ and fix an atomic set of blocks $\blocks$ for $u$ which induces the partial order $\bhb$. Assume that in $u$ for indices $i < j$, we have $i \not \bhb j$. Then, there exists a word $v \beq u$ and two indices $i' < j'$ such that $v[i']$ and $v[j']$ respectively are the same events as $u[j]$ and $u[i]$.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sabstract.tex <==
% !TEX root = ./main.tex

\begin{abstract}
\emph{Trace theory} (formulated by Mazurkiewicz in 1987) 
is a framework for designing equivalence relations for concurrent program runs
based on a commutativity relation over the set of atomic 
steps taken by individual program threads. 
It has been widely used in a variety of program verification and testing techniques. It is simple and elegant, and it yields efficient algorithms that are broadly useful in many different contexts. It is well-understood that the larger the equivalence classes are, the more benefits they would bring to the algorithms that use them. In this paper, we study relaxations of trace equivalence with the goal of maintaining its algorithmic advantages. We  prove that the largest appropriate relaxation of trace equivalence,  an equivalence relation that preserves the order of steps taken by each thread \emph{and} what write operation each read operation observes, does not yield efficient algorithms. Specifically, we prove a \emph{linear space lower bound} for the problem of checking if two arbitrary steps of a concurrent program run are \emph{causally concurrent} (i.e. they can be reordered in an equivalent run) or \emph{causally ordered }(i.e. they always appear in the same order in all equivalent runs). The same problem can be decided in \emph{constant space} for trace equivalence. 
\end{abstract}


==> sconclusion.tex <==
% !TEX root = ./main.tex

\section{Conclusion and Future Work}
We show that reads-from equivalence does not the nice algorithmic properties of (Mazurkiewicz) trace equivalence. On the theoretical side, it would be interesting to investigate whether there exists an equivalence relation that lies in between the two in terms of coarseness and yet retains these nice algorithmic properties. On the practical side, it would be interesting to investigate if non-constant space algorithms, for example those based on vector clocks, can still perform reasonably well in practice for reads-from equivalence.

==> serializability.tex <==
%!TEX root=./main.tex

\subsection{Serializability of Scattered Grains}

We next address the second challenge when incorporating
reasoning based on scattered grains.
Recall that, arbitrarily interleaved grains may never be brought together
and thus eligible to participate in swaps with other grains.
We therefore focus on scattered grains that are also \emph{serializable},
and formalize this intuition in the definition below:
% The precise definition of serializable we opt for uses $\rfnovaleq$ 
% We formalize this notion of consistency of a valid set of scattered grains as follows.

\begin{definition}[Serializability of Scattered Grains]
Let $\tr \in \alphabet$ be a run and let $\grains$ be a valid set of scattered grains in $\tr$.
We say that $\grains$ is serializable in $\tr$ if there is a run $\tr' \in \rfcl{\tr}$
such that $\grains$ is  a valid set of grains in $\tr'$ (in the sense of \defref{grain}).
\ucomment{Any other better definition?}
\end{definition}

\ucomment{Insert Theorem that says that checking serializability even for a single scattered grain is not constant space checkable. I guess if we choose $\ev{t_1, \wt(x_{\neg a_1})}$ and $\ev{t_2, \wt(u)}$ as the constituents of a scattered grain, then they can be brought together only when the blue events can be reordered.}

\begin{theorem}
The problem for checking if a given set $\grains$ of scattered grains 
is serializable in a given run $\tr$ cannot be solved using a streaming algorithm
that uses sub-linear space.
\end{theorem}

In light of our eventual goal of generalizing the formalism of \secref{beq}
to incorporate scattered grains based reasoning
in constant space, we draw inspiration from the notion of
\emph{conflict serializability} of transactions
from concurrency testing~\cite{Flanagan2008,FM08CAV} and inspired from
database concurrency control~\cite{}.
In the context of concurrency testing, this notion was shown to be 
monitorable in constant space~\cite{FM08CAV}.
In the context of scattered grains, the natural adaptation of this notion is the following.

\begin{definition}[Grain Conflict Serializability]
\deflabel{grain-conf-serial}
Let $\tr \in \alphabet$ be a run and let $\grains$ be a valid set of scattered grains in $\tr$.
$\grains$ is said to be grain conflict serialzable if
there is a run $\tr'$ such that $\tr' \mazeq \tr$ and each grain in $\grains$ appears
serially in $\tr$.
\end{definition}

\ucomment{In fig xxx, the set of grains is grain conflict serializable
because this other runs is maz equivalent to it and is also serial.}

The serializability notion we introduce (\defref{grain-conf-serial})
admits a graph based characterization, similar to the classic notion of 
conflict serializability~\cite{FM08CAV,Flanagan2008}.

\begin{lemma}
A set of grains $\grains$ is not grain conflict serializable in run $\tr$
iff there is a sequence $\grain_0, \grain_1 \ldots, \grain_{k-1}$ (with $k>1$)
and a sequence of events $e_0, f_0, e_1, f_1, \ldots, e_{k-1}, f_{k-1}$
such that for every $i$, $e_i \in \grain_i$, $f_i \in \grain_{(i+1)\% k}$
and $(e_i, f_i) \in \indrel$.
\end{lemma}

The overall design of our monitor for checking grain concurrency (\defref{gc})
relies on simultaneously \ucomment{guessing? the \emph{scattered grains}},
checking if they are grain conflict serializable
as well as checking concurrency.
Indeed grain conflict serializability can be checked in constant space,
if we restrict to grains that are also \emph{minimal}.
Recall that, this restriction is is without loss of generality (\lemref{minimal-grains-sufficient}).

\ucomment{Do we need to add a lemma saying that focusing on minimal grains also doesnt affect serializability. If we do, then perhaps we need to define an operation MINIMAL(G) that gives back the grains of G, but broken into minimal pieces.}



\subsection{Monitoring Grain Conflict Serializability}

We focus on scattered grains that are minimal (see \lemref{minimal-grains-sufficient}).
In this case, the number of scattered grains that are active
at any given prefix is bounded by $|\vars|$ (\lemref{minimal-grains-active-bound}).
We can therefore assume that the events of a given run are 
annotated with symbols
$\grainIDs = \set{1, 2, \ldots, |\vars|}$ denoting the grain identifier
they belong to, or alternatively with symbol $\unitgrain$ denoting events that do not belong to any grain.
Additionally the run contains demarcations $\bgn$ and $\egn$ denoting
start and end of grains.
Thus, the alphabet of runs can be assumed to be 
$\gMarkAlphabet = (\grainIDs \uplus \set{\unitgrain}) \times (\alphabet \uplus \set{\bgn, \egn})$.
% We remark that the following regular expression matches all \emph{well-formed}
% annotations:
% \[
% \Big((\unitgrain\times\alphabet) + \big((1,\bgn) (1\times\alphabet)^+ (1,\egn) + \cdots (|\vars|,\bgn) (i\times\alphabet)^+ (|\vars|,\egn)\big)\Big)^*
% \]

The choice of minimal grains and the resulting bound on the maximum
number of active grains lends itself to a \emph{summarized conflict graph} based
characterization of grain conflict serializability, similar to~\cite{FM08CAV}.
We define this graph next.
In the following, we use the notation $g \deadpath{\pi, \grains} g'$
to denote that there is a path from $g$ to $g'$ 
through \emph{dead} grains of a prefix $\pi$.
More formally, for prefix $\pi$ of run $\tr$, valid set of grains $\grains$
and grains (active or otherwise) $g, g'$ in $\pi$, 
we say that $g \deadpath{\pi, \grains} g'$ holds
if there are grains $\grain_1, \grain_2 \ldots, \grain_{k} \in \grains$ (with $k>1$, $g = g_1$ and $g' = g_{k}$) 
and events $e_1, f_1, e_2, f_2, \ldots, e_{k-1}, f_{k-1}$,
such that
$g_2, \ldots, g_{k-1} \subseteq \pi$ are dead (i.e., have started and completed) in $\pi$,
and $e_i \in g_i$, $f_i \in g_{i+1}$ and $(e_i, f_i) \in \deprel$ for $1 \leq i \leq k-1$.

\begin{definition}[Summarized Grain Conflict Graph]
Let $\tr$ be a run, $\grains$ be a valid set of scattered grains and let $\pi$ be a prefix of $\pi$.
The summarized conflict graph of $\pi$ is $G_\pi = (V_\pi, E_\pi, \contents_\pi, \summaries_\pi)$, where
\begin{enumerate}
	\item $V_\pi = \actv{\pi, \grains}$ is the set of active grains at the end of $\pi$,
	\item $(g, g') \in E_\pi$ if $g \deadpath{\pi, \grains} g'$,
	\item $\contents_\pi: V_\pi \to \powset{\alphabet}$ maps each active grain to  its current \emph{contents},
	i.e., $\contents_\pi(g) = \setpred{\tr[e]}{e \in g \cap \events{\pi}}$
	\item $\summaries_\pi: V_\pi \to \alphabet$ maps each active grain to the \emph{summaries} of
	dead grains, i.e.,
	$\summaries_\pi(g) = \setpred{\tr[e]}{\exists g' \subseteq \pi, g \deadpath{\pi, \grains} g', e \in g'}$.
\end{enumerate}
\end{definition}

We remark that summarized grain conflict graphs are sufficient to capture grain
conflict serializability:

\begin{lemma}
\lemlabel{summarized-acyclic}
Let $\tr$ be a run and let $\grains$ be a valid set of scattered grains in $\tr$.
$\grains$ is grain conflict serializable iff for every prefix $\pi$ of $\tr$,
the summarized conflict graph $G_\pi$ is acyclic.
\end{lemma}

\lemref{summarized-acyclic} will be crucially employed
in the monitor for grain conflict serializability, which
we describe next.

The states of our monitor are tuples $(V, E, C, S)$,
where $V \subseteq \grainIDs$, $E \subseteq V \times V$,
$C: V \to \powset{\alphabet}$ and $S: V \to \powset{\alphabet}$
and intuitively represent different summarized grain conflict graphs.
The transitions of the monitor can be described by the operator
$\sgup$ defined next.
Given $G = (V, E, C, S)$ and a symbol $b = (i, a) \in \gMarkAlphabet$,
the state $G' = (V', E', C', S') = G \sgup b$ can be described as follows:
\begin{description}
	\item[Case \underline{$i = \unitgrain$}.] In this case, $V' = V$,
	$E' = E$, $C' = C$ and for every $j \in V$,
	$S'(j) = S(j) \cup \setpred{a}{\exists a' \in C(j) \cup S(j), (a', a) \in \deprel}$

	\item[Case \underline{$i\in \grainIDs, a = \bgn$}.] In this case, $V' = V \uplus \set{i}$,
	$E' = E$, $C' = C$ and $S' = S$.

	\item[Case \underline{$i\in \grainIDs, a = \egn$}.] In this case, $V' = V \setminus \set{i}$,
	$E' = \proj{E}{V'} \cup \setpred{(j, k)}{(j, i) \in E, (i, k) \in E}$,
	$C' = \proj{C}{V'}$ and $S'$ is given as follows:
	$S'(i)$ is undefined, while for a $j \neq i$, $S'(j) = S(j)$ if $(j, i) \not\in E$,
	but $S'(j) = S(j) \cup C(i)$ otherwise.

	\item[Case \underline{$i\in \grainIDs, a \in \alphabet$}.] 
	In this case, $V' = V$,
	$E' = E \cup \setpred{(j, i)}{\exists a' \in C(j) \cup S(j), (a, a') \in \deprel}$,
	$C' = C \cup \set{a}$ and $S' = S$.
\end{description}
A state $(V, E, C, S)$ is rejecting if the transitive closure of $E$ is reflexive, i.e.,
there is a cycle in the graph $(V, E)$. All other states are accepting.

The transitions of the monitor are based on the following inductive
formalization of the summarized conflict graph:

\begin{lemma}
Let $\tr$ be a run and let $\grains$ be a valid set of minimal scattered grains in $\tr$.
Let $\pi$, $\pi'$ be prefixes of $\tr$ such that $\pi' = \pi \cdot e$ for some event $e$
such that $\tr[e] = (i, a)$, where $i \in \grainIDs \uplus \set{\unitgrain}$
and $a \in \alphabet$.
Then, $G_\pi' = (V_\pi, E_\pi, \contents_\pi, \summaries_\pi)$ is given by
$G' = G_\pi \odot \tr[e]$.
\end{lemma}

\begin{theorem}
Let $\tr$ be a \ucomment{annotated?} run  and let $\grains$ be a valid set of minimal scattered grains.
There is a constant space algorithm that checks if $\grains$
is grain conflict serializable.
\end{theorem}


==> sintro.tex <==
% !TEX root =  main.tex
\section{Introduction}
\seclabel{intro}


In the last 50 years, several models have been introduced for concurrency and parallelism, of which Petri nets \cite{hack1976petri}, Hoare's CSP \cite{hoare1978communicating}, Milner's CCS \cite{milner1980calculus}, and event structures \cite{Winskel1987} are prominent examples. Trace theory \cite{diekert1995book} is a paradigm in the same spirit which enriches the theory of words (or sequences) by a  very restricted yet wildly applicable mechanism to model parallelism:  a set of dependencies on {\em events} (atomic steps performed by individual threads) is determined statically, and any pair of sequences that can be transformed to each other through swaps of consecutive independent events are identified as {\em trace equivalent}. In other words, it constructs a notion of equivalence based on {\em commutativity} of individual events. The simplicity of trace theory, first formulated by Mazurkiewicz in 1987~\cite{Mazurkiewicz87}, has made it highly popular in a number of computer science areas, including programming languages, distributed computing, computer systems, and software engineering. It has been widely used in both dynamic program analysis and in construction of program proofs. In dynamic program analysis, it has add applications in predictive testing, for instance in data race prediction \cite{djit1999,Flanagan09,Elmas07,Smaragdakis12,Kini17} and in prediction of atomicity violation \cite{Farzan09,Sorrentino10,Farzan2006} among others. In verification, it is used for the inference of atomic blocks for local reasoning \cite{ElmasQT09,civl,KraglQH18}, or for the simplification of verification of concurrent and distributed programs \cite{mycav19,mypopl20,mypldi22,Genest07,psynch,Desai14}.


The brilliance of trace theory lies in its simplicity, both conceptually and in yielding simple and efficient algorithms for a collection of fundamental problems. The notion of equivalence put forward by trace theory yields simple efficient algorithms for several core problems in the context of concurrent and distributed programs. 
%Stateless Model Checking (SMC) \cite{Godefroid1997} is an effective verification technique for bounded concurrent programs. 
For instance, 
Dynamic Partial Order Reduction (DPOR) techniques  \cite{Flanagan2005,Kokologiannakis2022} are employed to reduce the number of program runs that must be explored to cover all possible program behaviours in Stateless Model Checking (SMC) \cite{Godefroid1997}. DPOR uses an equivalence relation over the program runs, such as trace equivalence, with the idea that it suffices to explore one run from each equivalence class. The same philosophy is employed in verification of arbitrary (not bounded) concurrent programs, when a proof is sought that covers at least one program behaviour from each equivalence class \cite{mycav19,mypopl20,mypldi22,Desai14,psynch,Genest07}. 

%The subprogram that is soundly proved correct in place of the original is called a {\em reduction}. In this context, the aim is for a simpler proof with simpler invariants. For example, in \cite{mycav19,mypopl20,mypldi22,Desai14,psynch,Genest07}, programs requiring complicated invariants can be automatically proved correct because the invariant of the reduction avoids these complications. 
%In \cite{Desai14,psynch,Genest07}, synchronous programs with simpler invariants serve as reductions of asynchronous programs with complex invariants that require reasoning about unbounded buffers. 

Since all the aforementioned application areas of trace theory (like DPOR) use a single representative in place of an entire set of equivalent runs, they would clearly benefit if larger sets of concurrent runs could soundly be considered equivalent. This motivates the key question in this paper: Can we retain all the benefits of classical trace theory while soundly enlarging the equivalence classes to improve the algorithms that use them? 
It is not difficult to come up with sound equivalence relations with larger classes. 
\citet{Abdulla2019} describe the sound equivalence relation, {\em reads-from equivalence}, which has the largest classes and is defined in a way to preserve two essential properties of 
\begin{wrapfigure}{r}{0.3\textwidth}
\vspace{-10pt}
\includegraphics[scale=0.75]{figures/intro-example}
\vspace{-10pt}
\caption{Read-From Equivalence}\label{fig:intro}
\vspace{-20pt}
\end{wrapfigure}
concurrent program runs: (1) the total order of {\em events} in each thread must remain the same in every equivalent run, 
and (2) each read event must observe the value written from the same write event in every equivalent run.   
%Let us consider the largest equivalence classes that remains sound (for most algorithms that use them) and maintain some other basic desirable properties. The corresponding equivalence relation, 
%called the {\em reads-from equivalence} in the literature~\cite{Abdulla2019},  is defined as one that preserves two essential properties from a concurrent program run: (1) the total order of {\em events} in each thread must remain the same in every equivalent run, and (2) each read event must observe the value written from the same write event in every equivalent run. 
The former is commonly referred to as the preservation of {\em program order}, 
and the latter as the preservation of the {\em reads-from} relation. These conditions guarantee that any equivalent run is also a valid run of the same concurrent program, and all the observed values (by read events) remain the same, which implies that the outcome of the program run must remain the same; in other words, control flow and data flow are preserved.



Consider the concurrent program run illustrated in \figref{intro}(a), and let us focus on the order of the events $\rd(x)$ from thread $T_1$ and $\wt(x)$ from thread $T_2$. In classical trace theory, these events are dependent (or \emph{conflicting}) and they must be ordered similarly in every equivalence class. This implies that the illustrated run belongs in an equivalence class of size 1. The situation is different if we were only concerned with preserving the reads-from relation.  A reads-from equivalent run is illustrated in \figref{intro}(b), in which the two events have been reordered. The arrows connect each write event to the read event that reads its value, which remain unchanged between the two runs.

We give a formal argument for why that the more relaxed reads-from equivalence is not as useful as trace equivalence from an algorithmic standpoint. One of the most fundamental algorithmic questions in this context is: Given two events $e$ and $e'$ in a run $\rho$, do they always appear in the same order in every member of the equivalence class of $\rho$ or can they be reordered in an equivalent run? In the former case, we call $e$ and $e'$ {\em causally ordered}, and otherwise {\em causally concurrent}.  For example, the events $\rd(x)$ from thread $T_1$ and $\wt(x)$ from thread $T_2$ are causally ordered under trace equivalence but are causally concurrent under reads-from equivalence. On the other hand, $\wt(z)$ event of thread $T_1$ and the $\rd(z)$ event of thread $T_2$ are causally ordered under both equivalence relations. 

%Consider the concurrent program run illustrate in \figref{intro}(a), and let us focus on the order of the events $\rd(x)$ from thread $T_1$ and $\wt(x)$ from thread $T_2$. In classic trace theory, these events are dependent and they must be ordered in every equivalence class. In the relaxed notion of equivalence that is only concerned with preserving the reads-from relation, however, they can be reordered.  The equivalent run that flips the order of these two events is illustrated in \figref{intro}(b). The (blue) arrows connect each write operation to the read operation that reads from it.
%
%Alternatively, consider the relative order of the $\wt(z)$ event of thread $T_1$ and the $\rd(z)$ event of thread $T_2$ in the run illustrated in \figref{intro}(a). Trace theory would declare the two events ordered and the verdict stands in reads-from equivalence as well, since the two events are bound by the reads-from relation.


For trace equivalence, it is possible to decide if two events are causally ordered or concurrent, using a {\em single pass constant space} algorithm; if the length of the run is assumed to be the size of the input, and other program measures such as the number of threads and the number of shared variables are considered to be constants. 
In \secref{semantic-equivalence}, we prove that if {\em equivalence} is defined as broadly as reads-from equivalence, then this check can no longer be done in {\em constant space} by proving a {\em linear space} lower bound (\thmref{check-order-semantic-linear-space-lower-bound}). In particular, we prove this for two closely related variation of this problem: (1) the decision is about the ordering of two specific events (as discussed in the example of \figref{intro}), and (2) the decision about the ordering of any two occurrences of a specific (atomic) action (e.g. are any two $\wt(x)$ actions unordered?). Both problems are closely related to predictive testing of violations of generic correctness properties for concurrent programs, such as data race freedom \cite{djit1999,Flanagan09,Elmas07,Smaragdakis12,Kini17} and atomicity \cite{Farzan09,Sorrentino10,Farzan2006}. With this, we can conclude that the more relaxed reads-from equivalence as amenable to algorithmic use as classical trace equivalence.





==> transitions-maz.tex <==
%!TEX root=./main.tex

\begin{figure}[t]
\begin{center}
\framebox{
\begin{minipage}{0.4\textwidth}
\begin{tabular}{lcl}
State & Event & State Update \\ \hline
$\langle-, E \rangle$ & $e \in \alphabet$ & $\langle -, E \rangle$ \\
$\langle -, E \rangle$ & $\focalEv_1$ & $\langle \focalEv_1, E \rangle$ \\
$\langle \focalEv_1, E \rangle$ & $e \in \alphabet$ & $\langle \focalEv_1 -, \{e\} \rangle$ \\
$\langle \focalEv_1 - , E \rangle$ & $e \in \alphabet$ & $\langle \focalEv_1 - , E \odot e \rangle$ \\
$\langle\focalEv_1 -, E \rangle$ & $\focalEv_2$ & $\langle \focalEv_1 - \focalEv_2, E \rangle$ \\
$\langle \focalEv_1 - \focalEv_2, E \rangle$ & $e \in \Sigma$ & $\langle \mathit{Ord}(E,e), E \rangle$ \\
%$\langle \mathit{true}, E \rangle$ & $e \in \Sigma$ &  $\langle a, E\rangle$\\
$\langle \mathit{false}, E \rangle$ & $e \in \Sigma$ &  $\langle \mathit{false}, E\rangle$\\
\end{tabular}
\end{minipage}
\begin{minipage}{0.4\textwidth}
%\begin{align*}
%E \odot \evt{\rd(x)}{i} &= \left\{ \begin{array}{ll}
%                                     E \cup \{\evt{\rd(x)}{i}\}  & \text{if }  \evt{\wt(x)}{i} \not \in E \\
%                                     E & \text{owise} 
%                                    \end{array}\right. \\
%E \odot \evt{\wt(x)}{i} &= E - \{\evt{\rd(x)}{i}\} \cup \{\{\evt{\wt(x)}{i}\}\}
%\end{align*}
\begin{align*}
E \odot e &= \left\{ \begin{array}{ll}
                                     E \cup \{e\}  & \text{if }  \exists e' \in E:\ (e,e') \in \deprel_\shasha \\
                                     E & \text{owise} 
                                    \end{array}\right.
\end{align*}
\begin{align*}
%\mathit{Ord}(E, \evt{\rd(x)}{i}) &\iff \evt{\wt(x)}{i} \in E  \\
%\mathit{Ord}(E, \evt{\wt(x)}{i}) &\iff \{\evt{\wt(x)}{i}, \evt{\rd(x)}{i}\} \cap E \not = \emptyset 
\mathit{Ord}(E, e) &\iff  \exists e' \in E:\ (e,e') \in \deprel_\shasha 
\end{align*}
\end{minipage}}\vspace{-5pt}
\caption{Trace Concurrency Monitor: The monitor starts in state $\langle -, \emptyset\rangle$ and accepts if in a state $\langle \mathit{false}, E\rangle$ (for any $E$) once the input is read. 
The operation $\odot$ updates a summary $E$ based on an new event. }
\label{fig:mcm}\vspace{-10pt}
\end{center}
\end{figure}
